MoCheQoS: Automated Analysis of Quality of Service Properties of Communicating Systems

We present MoCheQoS, a bounded model checker to analyse (QoS) properties of message-passing systems. Building on the dynamic temporal logic, the choreographic model, and the bounded model checking algorithm defined in our ICTAC 2023 paper, MoCheQoS enables the static analysis of QoS properties of systems built out from the composition of services. We consider QoS properties on measurable application-level attributes as well as resource consumption metrics for example those relating monetary cost to memory usage. The implementation of the tool is accompanied by an experimental evaluation. More precisely, we present two case studies meant to evaluate the applicability of MoCheQoS; the first is based on the AWS cloud while the second analyses a communicating system automatically extracted from code. Additionally, we consider synthetically generated experiments to assess the scalability of MoCheQoS. These experiments showed that our model can faithfully capture and effectively analyse QoS properties in industrial-strength scenarios.

==> affiliation.tex <==
\thanks{\tnxbehapi \tnxastra Carlos G.\ Lopez Pombo's research is
	 partly supported by Universidad de Buenos Aires by grant UBACyT
	 20020170100544BA and Agencia Nacional de Promoci\'on de la
	 Investigaci\'on, el Desarrollo Tecnol\'ogico y la Innovación
	 Científica through grant PICT-2019-2019-01793.
  	 \\[.5em]
	 The authors thank the anonymous reviewers for their constructive
	 comments.
	 \\[.5em]\
  }

\author{Carlos
  G. Lopez Pombo\thanks{On leave from CONICET-Universidad de Buenos Aires, Instituto de Ciencias de la Computaci\'{o}n, Buenos Aires, Argentina and Universidad de Buenos Aires, Facultad de Ciencias Exactas y Naturales, Departamento de Computaci\'{o}n, Buenos Aires, Argentina.
  }\inst{1}, Agust\'in E. Martinez Su\~n\'e\inst{2,3}, Emilio
  Tuosto\inst{4}
}
\institute{%
  Centro Interdisciplinario de Telecomunicaciones, Electrónica, Computación y Ciencia Aplicada - CITECCA, Universidad Nacional de Río Negro - Sede Andina, San Carlos de Bariloche, Argentina \\ \email{cglopezpombo@unrn.edu.ar} \and 
  CONICET-Universidad de Buenos Aires, Instituto de Ciencias de la Computaci\'{o}n, Buenos Aires, Argentina \and 
  Universidad de Buenos Aires, Facultad de Ciencias Exactas y Naturales, Departamento de Computaci\'{o}n, Buenos Aires, Argentina \\ \email{aemartinez@dc.uba.ar} \and
  Gran Sasso Science Institute, L'aquila, Italy \\   \email{emilio.tuosto@gssi.it}} 
\authorrunning{%
  Carlos G. Lopez Pombo, Agust\'in E. Martinez Su\~n\'e, Emilio Tuosto
}


==> analysis.tex <==
%!TEX root = ./main.tex

\SetKwFunction{qSat}{\textsc{qSat}}
\SetKwFunction{qModels}{\textsc{qModels}}
\SetKwFunction{qUntil}{\textsc{qUntil}}
\SetKwFunction{qRelease}{\textsc{qRelease}}
\SetKwFunction{traceOf}{\textsc{TraceOf}}

We now establish the semi-decidability of $\QL$ by presenting a
\mbox{$k$-bounded} semidecision procedure relying on three
algorithms: \qSat, \qModels, and \qUntil.
%
The \qSat algorithm is the main algorithm of the procedure and
determines whether a given formula is satisfiable in a given
system. It relies on \qModels to check if there is a run that
satisfies the formula which, in turn, uses \qUntil to handle the
$\qluntil[]$ operator.
%
Let us start by looking at \qSat defined as:%in \cref{alg:qsat}.
% 
%  It is important to note that while \qSat 
% guarantees a correct result when it terminates and returns true, 
% for an arbitrary formula, given the fixed bound $k$, it may return false
% even if the formula is satisfiable.
%
% \ \vspace{-20pt}

\begin{algorithm}[H]
  \scriptsize
% \caption{$k$-bounded semidecision procedure for $\QL$ satisfiability.} \label{alg:qsat}
\DontPrintSemicolon
\SetAlgoLined
% \KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
% \KwResult{Boolean indicating whether $\aCS \models \gqosprop$ holds or not.}
\SetKwProg{Fn}{}{\string:}{}
\Fn{\qSat{$\gqosprop,\aCS, k$}}
{
  $i = 0$\;
  \While{$i \leq k$}{
    \ForEach{$\pi \in \Delta_{\aCS}^i$}{
      \If{%
        the last configuration of $\pi$ is final and
        \qModels{$\gqosprop,\aCS,\pi,\epsilon$}
        \label{ln:qsat-qmodels}
      }{
        \Return{\textbf{true}}
      }
    }
    $i = i + 1$\;
  }
  \Return{\textbf{false}}
}
\end{algorithm}
% 
\noindent
Basically, \qSat enumerates all the runs of $\aCS$ up to a given bound
$k$ and checks whether any of them satisfies $\gqosprop$ (recall
that $\Delta_{\aCS}^i$ is the set of all runs of $\aCS$ with length
$i$).
%  The algorithm returns false if there is no run in $\aCS$ of length up to $k$ satisfying $\gqosprop$.
Let us now focus on the algorithm \qModels:% (cf. \cref{alg:qmodels}).
%
% \ \vspace{-20pt}

\begin{algorithm}[H]
  \scriptsize
% \caption{Decision procedure for the satisfaction relation of $\QL$}\label{alg:qmodels}
\DontPrintSemicolon
\SetAlgoLined
% \KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
% \KwResult{Boolean indicating whether $\aCS \models \gqosprop$ holds or not.}
\SetKwProg{Fn}{}{\string:}{}
\Fn{\qModels{$\gqosprop,\aCS,\pi,\pi'$}}
{
  % \SetInd{before space}{after space}
  % \KwData{$\pi'$ is of the form $q_0\ \TRANSS{\al_1} \dots \TRANSS{\al_n}\ q_n$}
  \Switch{$\gqosprop$}{
  \Case{$\top$}{
    \Return{\textbf{true}}
    \label{ln:qsat-true}
  }
  \Case{$\psi$}{
    \Return{
      whether $\aggfn_{\aCS} (\pi') \vdash_{\mathit{RCF}} \psi$
    }
    \label{ln:qsat-rcf}
  }
  % \lnl{ln:neg}
  \Case{$\neg\gqosprop_1$}{
    \Return{\textbf{\emph{not}} \qModels{$\gqosprop_1,\aCS,\pi,\pi'$}}
  }
  \Case{$\gqosprop_1 \lor \gqosprop_2$}{
    \Return{\qModels{$\gqosprop_1,\aCS,\pi,\pi'$} \textbf{\emph{or}} \qModels{$\gqosprop_2,\aCS,\pi,\pi'$}}
    \label{ln:qsat-or}
  }
  \Case{$\gqosprop_1\ \qluntil\ \gqosprop_2$}{
    \Return{\qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi',\epsilon$}}
    \label{ln:qsat-until}
  }
        % \lnl{4}\lIf{\qModels{$\gqosprop_2,\aCS,\pi'$}}{\Return{\textbf{true}}}
        %          \Else{
        %       \lnl{5}\ForEach{$\aConf \TRANSS{\al} \aConf'$ on $\aCS$}{
        %             \lnl{6}\lIf{\qModels{$\gqosprop_1,\aCS,\pi'$} \textbf{\emph{and}} $(  \mathcal{L}(\pi' \cdot \aConf \TRANSS{\al} \aConf') \in \rlang[\aG]$ $\&\&$ \qModels{$\gqosprop_1\ \qluntil\ \gqosprop_2,\aCS, \pi' \cdot \aConf \TRANSS{\al} \aConf'$})}{\Return{\textbf{true}}}}
        %             \lnl{7}\Return{\textbf{false}}
        %          }
  }
}
\end{algorithm}
% 
\noindent
Following \cref{def:ql-semantics}, \qModels recursively inspects the
$\QL$ formula. It invokes 
\qUntil to handle the $\qluntil[]$ operator
and the decision procedure of the theory of real-closed fields to
check the atomic formulae.
Let us now look at the algorithm \qUntil:% in \cref{alg:quntil}.
%
% \ \vspace{-20pt}

\begin{algorithm}[H]
  \scriptsize
% \caption{Auxiliary decision procedure for the $\qluntil$ operator.}\label{alg:quntil}
\DontPrintSemicolon
\SetKwProg{Fn}{}{\string:}{}
\Fn{\qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''$}}
{
  % \KwData{$\pi''$ is of the form $q_0\ \TRANSS{} \dots \TRANSS{}\ q_n$}
  \If{$\rlang[\pi''] \in \hat{\rlang}[\aG]$ and $\qModels{$\gqosprop_2,\aCS,\pi,\pi'\pi''$}$
    \label{ln:quntil-base-true-condition}
  }
  {
    \Return{\textbf{true}}
    \label{ln:quntil-base-true}
  }
  \ElseIf{not \qModels{$\gqosprop_1,\aCS,\pi,\pi'\pi''$}
    \label{ln:quntil-base-false-condition}
  }
  {
    \Return{\textbf{false}}
    \label{ln:quntil-base-false}
  }
  \Else{
    % \label{ln:}
    % Let $\mathcal{N}$ be the set $\set{\pi''\ \TRANSS{\al}\ q \in \Delta_{\aCS} \sst \mathcal{L}(\pi''\ \TRANSS{\al}\ q) \in \mathit{prf}(\rlang[\aG])}$\\
    Let $\TRANSS{\al}\ q$ be the transition such that $\pi'\pi''\ \TRANSS{\al}\ q \in \mathit{prf}(\pi)$
    \label{ln:quntil-transition}
    \newline (takes the first transition in $\pi$ if $\pi'\pi'' = \epsilon$,
    \newline and it is not defined if $\pi'\pi'' = \pi$)\;
    \If{$\pi'\pi'' = \pi$ or $\rlang[\pi''\ \TRANSS{\al}\ q] \not\in \rlang[\aG]$}{
      \Return{\textbf{false}}
      \label{ln:quntil-empty-false}
    }
    \Else
    % {%$\mathcal{L}(\pi''\ \TRANSS{\al}\ q) \in \mathit{prf}(\rlang[\aG])$
    % \label{ln:quntil-recursive-condition}
    % }
    {
      \Return{\qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''\ \TRANSS{\al}\ q$}}
      \label{ln:quntil-recursive}
    }
    % \Else{
    %   \Return{\textbf{false}}
    %   \label{ln:quntil-recursive-false}
    % }
  }
}
% \lnl{ln:quntil-false}
\end{algorithm}
% 
\noindent
This procedure takes care of searching for a witness of the
existential in the semantics of $\qluntil[]$ by starting in the
current prefix $\pi'$ and following the transitions of $\pi$.
% Let's now shift our focus to \cref{alg:quntil}, which implements \qUntil.
According to \cref{def:ql-semantics}, \qUntil searches for a witness of the
existential part of $\qluntil[]$.
%
It takes as parameters the complete run $\pi$, the prefix $\pi'$ at
which the $\qluntil[]$ is being evaluated, and the current extension
$\pi''$ that is used to search for the witness.
%
If $\pi''$ is enough to reach a verdict, the algorithm returns true or
false accordingly (\cref{ln:quntil-base-true,ln:quntil-base-false}).
%
Otherwise, it tries to extend $\pi''$ by borrowing the next transition
of $\pi$ (\cref{ln:quntil-transition}).
%
If such extension exists and is a candidate for being in the language
of $\aG$, the algorithm recursively calls itself with the extended
prefix (\cref{ln:quntil-recursive}).
% 
Hereafter, we fix a QoS-extended communicating system $\aCS$.

\begin{theorem}[\qSat is sound and $k$-bounded complete]
  \label{lem:qsat}
  Given a QoS formula $\gqosprop \in \QL$ and a bound $k$,
  % \begin{center}
    \qSat{$\gqosprop, \aCS,k$} returns \textbf{true} iff
    there exists $\pi \in \Delta^i_{\aCS}$ such that
    $\conf{\pi, \epsilon} \models_{\aCS} \gqosprop$,
    for some $i \leq k$.
  % \end{center}
\end{theorem}
The soundness of \qSat immediately follows from the soundness of \qModels
(established in \cref{lem:qmodels} below) which, in turn, relies on the
soundness and completeness of \qUntil (cf.
\cref{lem:quntil-correct,lem:quntil-complete}, respectively).
%
This guarantees that the call to \qModels in \cref{ln:qsat-qmodels} of
\qSat returns true iff the run $\pi$ satisfies $\gqosprop$.
%
Note that \qSat is not guaranteed to be complete due to the bound
$k$.

\begin{lemma}[\qModels\ is sound and complete]
  \label{lem:qmodels}
  Given a QoS formula $\gqosprop \in \QL$ and runs $\pi, \pi' \in \Delta_{\aCS}$, 
  where $\pi' \in \mathit{prf}(\pi)$,
  % \begin{center}
    \qModels{$\gqosprop, \aCS,\pi,\pi'$} returns \textbf{true} iff $\conf{\pi, \pi'} \models_{\aCS} \gqosprop$.
  % \end{center}
\end{lemma}

\begin{proof}
  By structural induction on $\gqosprop$.
  %
  If $\gqosprop$ is $\top$, 
  % the algorithm returns true and 
  the result follows trivially.
  %
  If $\gqosprop$ is an atomic formula, the algorithm computes the
  aggregation over the run $\pi'$ (\cref{ln:qsat-rcf}) and invokes the
  decision procedure of RCFs to check whether $\aggfn_{\aCS} (\pi')$ entails
  $\gqosprop$ in the theory of real closed fields.
  %
  If $\gqosprop$ is $\gqosprop_1 \lor \gqosprop_2$, the algorithm perform two recursive calls and returns true iff either $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1$ or $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_2$. %Which is equivalent to $\exists \pi \in \Delta^\infty_{\aCS}$ such that either $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1$ or $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_2$.
  % If $\gqosprop$ is $\gqosprop_1 \land \gqosprop_2$, the algorithm perform two recursive calls and returns true iff both $\exists \pi_1 \in \Delta^\infty_{\aCS}$ such that $\conf{\pi_1, \pi'} \models_{\aCS} \gqosprop_1$ and $\exists \pi_2 \in \Delta^\infty_{\aCS}$ such that $\conf{\pi_2, \pi'} \models_{\aCS} \gqosprop_2$. We need to show that $\exists \pi \in \Delta^\infty_{\aCS}$ such that $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1$ and $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_2$ \anote{What guarantees $\pi_1 = \pi_2$?}.
  If $\gqosprop$ is $\gqosprop_1\ \qluntil\ \gqosprop_2$, the algorithm returns true iff \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \epsilon$} returns true. By \cref{lem:quntil-correct,lem:quntil-complete} this is equivalent to $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1\ \qluntil\ \gqosprop_2$.
  % Cases $\top$ and $\bot$ are trivial.
\qed
\end{proof}

We now prove the soundness and completeness of \qUntil.

\begin{lemma}[\qUntil\ is sound]
  \label{lem:quntil-correct}
  Given a QoS formula $\gqosprop_1, \gqosprop_2 \in \QL$, a
  g-choreography $\aG$, and runs $\pi, \pi', \pi''$ such that
  \begin{enumerate}[label = \alph*)] 
  \item
    \label{lem:quntil-correct:hyp-runs-in-sys}
    $\pi'\pi'' \in \mathit{prf}(\pi)$ and $\pi \in \Delta_{\aCS}$, and 
    % \item 
    % \label{lem:quntil-correct:hyp2}
    % $\rlang[\pi''] \in \mathit{prf}(\rlang[\aG])$, 
  \item
    \label{lem:quntil-correct:hyp-prefixes}
    for all $\pi''' \in \mathit{prf}(\pi'')$, if $\pi''' \neq \pi''$ then 
    % $\neg\left(\rlang[\pi'''] \in \rlang[\aG] \land \exists \pi \in \Delta^\infty_{\aCS} \conf{\pi, \pi'\pi'''} \models_{\aCS} \gqosprop_2 \right)$ and 
    $\conf{\pi, \pi'\pi'''} \models_{\aCS} \gqosprop_1$
    % \item 
  \end{enumerate}
  % then
  % \begin{center}
  if \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''$}
  returns \textbf{true}
  % \\
  then
  $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1\ \qluntil\
  \gqosprop_2$.
  % \end{center}
\end{lemma}
%
\begin{proof}
  The call to
  \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''$} either
  reaches \cref{ln:quntil-base-true} or it reaches \cref{ln:quntil-recursive}
  and the recursive call returns true.  In the first case, we know
  % that 
  $\rlang[\pi''] \in \hat{\rlang}[\aG]$ and that
  $\qModels{$\gqosprop_2,\aCS,\pi,\pi'\pi''$}$ returned true.  By
  \cref{lem:qmodels} it follows that
  $\conf{\pi, \pi'\pi''} \models_{\aCS} \gqosprop_2$.  Together with
  hypotheses \ref{lem:quntil-correct:hyp-runs-in-sys} and
  \ref{lem:quntil-correct:hyp-prefixes} the conditions of the
  semantics of the formula $\gqosprop_1\ \qluntil\ \gqosprop_2$
  (see \cref{def:ql-semantics}) are met.  In the case of reaching
  \cref{ln:quntil-recursive} we know the recursive call
  \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''\
	 \TRANSS{\al}\ q$} returned true.  
  %  Notice that 
   Conditions
  \ref{lem:quntil-correct:hyp-runs-in-sys} and
  \ref{lem:quntil-correct:hyp-prefixes} applied to the input of the
  recursive call holds because of the way transition $\TRANSS{\al}\ q$
  was chosen and the fact that condition on
  \cref{ln:quntil-base-false-condition} returned false.  Therefore, we
  can take the output of the recursive call to satisfy
  \cref{lem:quntil-correct} as an inductive hypothesis and conclude
  $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1\ \qluntil\
  \gqosprop_2$.
  % It only remains to notice that $\pi'\pi'' \in \mathit{prf}(\pi)$, which can be derived from $\pi'\pi'' \in \mathit{prf}(\pi'\pi''\ \TRANSS{\al}\ q)$ and $\pi'\pi''\ \TRANSS{\al}\ q \in \mathit{prf}(\pi)$.
\qed
\end{proof}

\begin{lemma}[\qUntil is complete]
  \label{lem:quntil-complete}
  Given a QoS formula $\gqosprop_1, \gqosprop_2 \in \QL$, a g-choreography $\aG$, and runs $\pi, \pi', \pi''$ such that 
  \begin{enumerate}[label = \alph*)] 
    \item 
    \label{lem:quntil-complete:hyp-runs-in-sys}
    $\pi'\pi'' \in \mathit{prf}(\pi)$ and $\pi \in \Delta_{\aCS}$, and 
    \item 
    \label{lem:quntil-complete:hyp-prefixes}
    for all $\pi''' \in \mathit{prf}(\pi'')$, if $\pi''' \neq \pi''$ then 
    either $\rlang[\pi'''] \not\in \hat{\rlang}[\aG]$ or $\conf{\pi, \pi'\pi'''} \nvDash_{\aCS} \gqosprop_2$
    % $\exists \pi \in \Delta^\infty_{\aCS} \conf{\pi, \pi'\pi'''} \models \gqosprop_1$
  \end{enumerate}
  % then
  % \begin{center}
    if \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''$} returns \textbf{false}
    then $\conf{\pi, \pi'} \nvDash_{\aCS} \gqosprop_1\ \qluntil\ \gqosprop_2$
  % \end{center}
\end{lemma}

\begin{proof}
  The call to \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''$} reaches either \cref{ln:quntil-base-false}, \cref{ln:quntil-empty-false} or it reaches \cref{ln:quntil-recursive} and the recursive call returns false.
  % 
  In all cases, by condition \ref{lem:quntil-complete:hyp-prefixes} we know that no prefix of $\pi''$ could be witness of the existential in the semantics of $\gqosprop_1\ \qluntil\ \gqosprop_2$ (see \cref{def:ql-semantics}) because it would need to both be in $\hat{\rlang}[\aG]$ and satisfy $\gqosprop_2$. Run $\pi''$ itself cannot be the witness for the same reasons due to the fact that condition in \cref{ln:quntil-base-true-condition} was not met. Which means either $\rlang[\pi''] \not\in \hat{\rlang}[\aG]$ or $\qModels{$\gqosprop_2,\aCS,\pi,\pi'\pi''$}$ returned false, therefore, using \cref{lem:qmodels}, either $\rlang[\pi''] \not\in \hat{\rlang}[\aG]$ or $\conf{\pi, \pi'\pi''} \nvDash_{\aCS} \gqosprop_2$.
  The only remaining possibility is for the witness to be a $\pi^\star$ such that $\pi'' \in \mathit{prf}(\pi^\star)$ and
  $\pi^\star \neq \pi''$.
  % 
  In the case of reaching \cref{ln:quntil-base-false}, we know that \qModels{$\gqosprop_1,\aCS,\pi,\pi'\pi''$} returned false. 
  By \cref{lem:qmodels} it follows that $\conf{\pi, \pi'\pi''} \nvDash_{\aCS} \gqosprop_1$.
  Therefore, extension $\pi^\star$ couldn't be a witness for the existential in the semantics of $\gqosprop_1\ \qluntil\ \gqosprop_2$.
  % 
  In the case of reaching \cref{ln:quntil-empty-false}, candidate extension $\pi^\star$ does not exist or it is not in $\hat{\rlang}[\aG]$.
  % 
  In the case of reaching \cref{ln:quntil-recursive}, we know that \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi,\pi', \pi''\ \TRANSS{\al}\ q$} returned false.
  Notice that conditions
  \ref{lem:quntil-complete:hyp-runs-in-sys} and 
  \ref{lem:quntil-complete:hyp-prefixes} applied to the input of the recursive calls holds because
  of the way transition $\TRANSS{\al}\ q$ was chosen and
  that condition in \cref{ln:quntil-base-true-condition} was not met.
  Therefore, we can take the output of the recursive calls to satisfy \cref{lem:quntil-complete} as an inductive hypothesis and conclude that $\conf{\pi, \pi'} \nvDash \gqosprop_1\ \qluntil\ \gqosprop_2$.
  % This discards any candidate extension $\pi^\star$
  %  in the set $\set{\pi''' \sst \pi''\ \TRANSS{\al}\ q \in \mathit{prf}(\pi''') \land \pi''\ \TRANSS{\al}\ q \in \mathcal{N}}$.
  % Any $\pi'''$ extension of $\pi''$ outside this set fails to be a witness for the existential in the semantics of $\gqosprop_1\ \qluntil\ \gqosprop_2$ because $\rlang[\pi'''] \not\in \rlang[\aG]$ due to the way $\mathcal{N}$ is built.
\qed
\end{proof}
Notice that the proof for \cref{lem:qmodels} uses \cref{lem:quntil-complete}
and \cref{lem:quntil-correct}, and that the proofs for \cref{lem:quntil-complete}
and \cref{lem:quntil-correct} use \cref{lem:qmodels}.
This does not undermine the soundness of the proofs because the lemmas are 
always (inductively) applied on smaller $\QL$ formulas.
Now that the soundness and completeness of \qModels and \qUntil is established, 
it remains to show their termination. Termination follows from the fact that
both the number of logical operators in $\gqosprop$ and the number of transitions in $\pi$ are finite.
The first guarantees \qModels eventually reaches a base case and the second guarantees \qUntil eventually 
reaches a base case.
Finally, the base case in \qModels, computing aggregation and checking entailment in the theory of real closed 
fields, terminates due to the decidability of RCFs \cite{tarski:RM-109}.
% Finally, the base case in \qModels that computes the aggregation and checks entailment in the theory of real closed 
% fields is guaranteed to terminate because RCFs are decidable \cite{tarski:RM-109}.

\subsection{A bounded model-checking approach for $\QL$}

Previous results allow for a straightforward bounded
model-checking approach for $\QL$.  Like for other model-checking
procedures for a language that admits negation, \qSat\ can be used to
check validity of a $\QL$ formula in a system $\aCS$ by checking the
satisfiability of the negated formula. This constitutes a
counterexample-finding procedure for $\QL$. The caveat is that
\qSat is a $k$-bounded semidecision procedure rather than a decision
procedure.  However, restricting to $\QL^-$, namely $\QL$ formulae
that do not contain the $\grecop$ operator in their choregraphies, we
 can find finite models of satisfiable formulae of $\QL^-$
(cf. \cref{lem:fmp}). 
% Thus, \qSat can serve as a
% decision procedure for $\QL^-$, if one computes a
% suitable bound $k$.

% \begin{lemma}[Termination of \qModels]
%   \label{lem:termination}
%   Given a QoS-extended communicating system $\aCS$, a QoS formula $\gqosprop \in \QL$ and a run $\pi' \in \Delta_{\aCS}$, the execution of \qModels{$\gqosprop, \aCS, \pi'$} finishes in a finite amount of steps.
% \end{lemma}

% \begin{proof}
%   Let $\mathit{max\_trace}(\gqosprop)$ be the maximum of the set $\set{ \text{length of }\pi \sst \mathcal{L}(\pi) \in \rlang[\aG], \aG \text{ appears in } \gqosprop}$. Notice that, since every $\aG$ considered does not contain $\grecop$, $\mathit{max\_trace}$ is finite. Let $\mathit{ops}(\gqosprop)$ be number of logical operators involved in $\gqosprop$. Let $\mathit{len}(\pi)$ be the number of transitions in $\pi$.
%   Let the metric $m$ over the inputs be defined as follows:
%   $$
%   m(\gqosprop, \pi') = \mathit{ops}(\gqosprop) + \mathit{max\_trace}(\gqosprop) - \mathit{len}(\pi')
%   $$
%   For \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi', \pi''$} and \qRelease{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi', \pi''$} we'll consider $m(\gqosprop_1\ \qluntil\ \gqosprop_2,\ \pi'\pi'')$ and $m(\gqosprop_1\ \mathcal{R}^{\aG}\ \gqosprop_2,\ \pi'\pi'')$ respectively.

%   All \qModels, \qUntil and \qRelease are recursive. A call to any one of them yields a series of direct recursive calls and indirect recursive calls that might involve the other two. We'll show that any recursive call in \qModels, \qUntil or \qRelease, be it direct or indirect, decreases $m$.
%   First consider \qModels, direct recursive calls in it (\cref{ln:qsat-and,ln:qsat-or}) decrease $m$ because they decrease $\mathit{ops}(\gqosprop)$ by at least one, mantain $\mathit{len}(\pi')$ constant and might decrease $\mathit{max\_trace}(\gqosprop)$.
%   Calls to \qUntil and \qRelease in \qModels (\cref{ln:qsat-until,ln:qsat-release}) do not change $m$ but, as we'll see in the following, any call inside \qUntil or \qRelease necessarily decreases $m$.
%   Consider now \qUntil, direct recursive calls in it (\cref{ln:quntil-recursive-condition}) decrease $m$ because they maintain $\mathit{ops}(\gqosprop)$, increase $\mathit{len}(\pi')$ by one and maintain $\mathit{max\_trace}(\gqosprop)$.
%   Calls to \qModels inside \qUntil (\cref{ln:quntil-base-true-condition,ln:quntil-base-false-condition}) decreases $m$ because it decreases $\mathit{len}(\gqosprop)$ by at least one, might increase $\mathit{len}(\pi')$ and might decrease $\mathit{max\_trace}(\gqosprop)$.
%   The reasoning for direct recursive calls in \qRelease(\cref{ln:qrelease-recursive-true-condition}) and calls to \qModels insinde \qRelease (\cref{ln:qrelease-base-true-condition,ln:qrelease-base-false-condition}) is analogous.

%   By definition, neither $\mathit{ops}(\gqosprop)$ nor $\mathit{max\_trace}(\gqosprop)$ can be negative. Therefore, if $m(\gqosprop, \pi')$ reaches zero, then both $\mathit{ops}(\gqosprop) = 0$ and $\mathit{max\_trace}(\gqosprop) = \mathit{len}(\pi')$. The first condition implies that a base case in \qModels was reached, while the second condition implies that base cases in \qUntil and \qRelease were reached because there is no way to extend $\pi'$ for it to be inside the language of any $\aG$ in the formula. In any case, the algorithm terminates.
  
%   It remains to argue that \qModels base case in \cref{ln:qsat-rcf} is guaranteed to terminate and that the number of direct recursive calls inside \qUntil(\cref{ln:quntil-recursive}) and \qRelease(\cref{ln:qrelease-recursive-true}) is finite.
%   The first follow from the decidability of RCFs\cite{tarski:RM-109} and the second from the fact that the number of transitions in $\aCS$ is finite.
%\qed 
% \end{proof}

\begin{theorem}[Finite model property of $\QL^-$]
  \label{lem:fmp}
  Given a QoS formula $\gqosprop \in \QL^-$, and runs $\pi \in \Delta_{\aCS}^\infty$, $\pi' \in \Delta_{\aCS}$ such that $\pi' \in \mathit{prf}(\pi)$.
  If $\conf{\pi, \pi'} \models_{\aCS} \gqosprop$ then there exists a finite run $\pi^- \in \Delta_{\aCS}$ such that $\pi^- \in \mathit{prf}(\pi)$ and $\conf{\pi^-, \pi'} \models_{\aCS} \gqosprop$.
\end{theorem}

\begin{proof}
  By structural induction on $\gqosprop$.
  If $\gqosprop$ is $\top$ or an atomic formula, take $\pi^- = \pi'$.
  If $\gqosprop$ is $\gqosprop_1 \lor \gqosprop_2$, we have that either $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_1$ or $\conf{\pi, \pi'} \models_{\aCS} \gqosprop_2$. 
  By inductive hypothesis, either $\conf{\pi_1^-, \pi'} \models_{\aCS} \gqosprop_1$ or $\conf{\pi_2^-, \pi'} \models_{\aCS} \gqosprop_2$ for some finite $\pi_1^-,\pi_2^- \in \mathit{prf}(\pi)$. 
  Therefore, either $\conf{\pi_1^-, \pi'} \models_{\aCS} \gqosprop_1 \lor \gqosprop_2$ or $\conf{\pi_2^-, \pi'} \models_{\aCS} \gqosprop_1 \lor \gqosprop_2$.
  
  If $\gqosprop$ is $\gqosprop_1\ \qluntil\ \gqosprop_2$, by \cref{def:ql-semantics} we have there exists $\pi''$ such that $\rlang[\pi''] \in \rlang[\aG]$,
   $\pi'\pi'' \in \mathit{prf}(\pi)$ up to a final configuration
   with $\conf{\pi, \pi'\pi''} \models_{\aCS} \gqosprop_2$, and for all $\pi''' \in \mathit{prf} (\pi'')$, if $\pi''' \neq \pi''$ then $\conf{\pi, \pi'\pi'''} \models_{\aCS} \gqosprop_1$.
  If we apply the inductive hypothesis to $\gqosprop_1$ and $\gqosprop_2$, we have
  there exists $\pi''$ such that $\rlang[\pi''] \in \rlang[\aG]$,
  $\pi'\pi'' \in \mathit{prf}(\pi)$ up to a final configuration
  with $\conf{\pi_2^-, \pi'\pi''} \models_{\aCS} \gqosprop_2$ for some 
  $\pi_2^- \in \Delta_{\aCS}$ such that 
  $\pi_2^- \in \mathit{prf}(\pi)$, and for all $\pi''' \in \mathit{prf} (\pi'')$, if $\pi''' \neq \pi''$ then  $\conf{\pi_1^-, \pi'\pi'''} \models_{\aCS} \gqosprop_1$ for some 
  $\pi_1^- \in \Delta_{\aCS}$ such that 
  $\pi_1^- \in \mathit{prf}(\pi)$. 
  % If we apply the inductive hypothesis to $\gqosprop_1$ and $\gqosprop_2$, we have there exists $\pi''$ such that $\pi'\pi'' \in \mathit{prf}(\pi)$ and $\rlang[\pi''] \in \rlang[\aG]$, and $\conf{\pi_2^-, \pi'\pi''} \models_{\aCS} \gqosprop_2$ for some 
  % $\pi_2^- \in \Delta_{\aCS}$ such that 
  % $\pi_2^- \in \mathit{prf}(\pi)$, and for all $\pi''' \in \mathit{prf} (\pi'')$, if $\pi''' \neq \pi''$ then $\conf{\pi_1^-, \pi'\pi'''} \models_{\aCS} \gqosprop_1$ for some 
  % % $\pi_1^- \in \Delta_{\aCS}$ such that 
  % $\pi_1^- \in \mathit{prf}(\pi)$. 
  Notice that since $\aG$ is $\grecop$-free, run $\pi''$ in the language $\rlang[\aG]$ is necessarily finite
  and so is the number of quantified runs $\pi'''$.
  Therefore, the number of runs $\pi_1^-$ involved in the previous statement is finite, and there is a maximum among their lengths,
  so we can take $\pi^-$ as the longest between $\pi_2^-$ and runs $\pi_1^-$.
  Since $\pi_2^-$ and all the $\pi_1^-$ are prefixes of $\pi$, then they will also be prefixes of $\pi^-$, and therefore we have the conditions to conclude $\conf{\pi^-, \pi'} \models_{\aCS} \gqosprop_1\ \qluntil\ \gqosprop_2$.
  
  If the outermost operator in $\gqosprop$ is $\neg$, we need to consider al the possible cases for the immediate subformula of $\gqosprop$.
  If $\gqosprop$ is $\neg\psi$ with $\psi$ atomic formula, we have that $\conf{\pi, \pi'} \nvDash_{\aCS} \psi$. 
  Take $\pi^- \in \mathit{prf}(\pi)$ an extension of $\pi'$ whose last configuration is final.
  % It follows that $\conf{\pi', \pi'} \nvDash_{\aCS} \psi$ and we can take $\pi^- = \pi'$.
  If $\gqosprop$ is $\neg(\gqosprop_1 \lor \gqosprop_2)$, we have that $\conf{\pi, \pi'} \nvDash_{\aCS} \gqosprop_1 \lor \gqosprop_2$. It follows that $\conf{\pi, \pi'} \nvDash_{\aCS} \gqosprop_1$ and $\conf{\pi, \pi'} \nvDash_{\aCS} \gqosprop_2$. By inductive hypothesis, there exists $\pi_1^- \in \Delta_{\aCS}$ such that $\pi_1^- \in \mathit{prf}(\pi)$ and $\conf{\pi_1^-, \pi'} \nvDash_{\aCS} \gqosprop_1$ and there exists $\pi_2^- \in \Delta_{\aCS}$ such that $\pi_2^- \in \mathit{prf}(\pi)$ and $\conf{\pi_2^-, \pi'} \nvDash_{\aCS} \gqosprop_2$. It is enough to take $\pi^-$ as the longest between $\pi_1^-$ and $\pi_2^-$.
  If $\gqosprop$ is $\neg(\gqosprop_1\ \qluntil\ \gqosprop_2)$, we have that $\conf{\pi, \pi'} \nvDash_{\aCS} \gqosprop_1\ \qluntil\ \gqosprop_2$. Therefore, for all $\pi''$ such that $\pi'\pi'' \in \mathit{prf}(\pi)$ up to a final configuration of $\pi$, if $\rlang[\pi''] \in \rlang[\aG]$, and $\conf{\pi, \pi'\pi''} \models_{\aCS} \gqosprop_2$, then there exists $\pi''' \in \mathit{prf} (\pi'')$, with $\pi''' \neq \pi''$ such that $\conf{\pi, \pi'\pi'''} \models_{\aCS} \neg\gqosprop_1$.
  If we apply the inductive hypothesis to $\gqosprop_2$ and $\neg\gqosprop_1$, we have that for all $\pi''$ such that $\pi'\pi'' \in \mathit{prf}(\pi)$ up to a final configuration of $\pi$, if $\rlang[\pi''] \in \rlang[\aG]$, and $\conf{\pi_2^- , \pi'\pi''} \models_{\aCS} \gqosprop_2$ for some $\pi_2^- \in \Delta_{\aCS}$ with $\pi_2^- \in \mathit{prf}(\pi)$, then there exists $\pi''' \in \mathit{prf} (\pi'')$, with $\pi''' \neq \pi''$ such that $\conf{\pi_1^-, \pi'\pi'''} \models_{\aCS} \neg\gqosprop_1$ for some $\pi_1^- \in \Delta_{\aCS}$ with $\pi_1^- \in \mathit{prf}(\pi)$. Notice that since $\aG$ is $\grecop$-free, any run in the language $\rlang[\aG]$ is necessarily finite. Therefore, there is a maximum among the lengths of the runs $\pi_2^-$, and we can take $\pi^-$ as the longest between $\pi_2^-$ and $\pi_1^-$.
\qed
\end{proof}

The proof of Thm.~\ref{lem:fmp} hints that the length of the 
run $\pi^-$ constitutes a suitable bound for \qSat;
% That is, recursively in the structure of $\gqosprop$ by taking the maximum between the bounds of the immediate subformulae and, for the case of the $\qluntil$ operator, the length of the longest run in $\rlang[\aG]$. 
which would turn \qSat into a decision procedure for $\QL^-$ 
if one could compute such bound.
Searching for counterexamples of an arbitrary formula $\gqosprop \in \QL$ up to a bounded number of unfoldings
of 
% the 
$\grecop$ 
% operator 
is equivalent to searching for counterexamples in a formula $\hat \gqosprop$ in $\QL^-$ where each 
$\grecop$ 
% operator 
has been replaced by a finite number of unfoldings. 
% Which means that the bound 
% % computed
% for models of formulae in $\QL^-$ could be used to search for counterexamples of formulae 
% in $\QL$.
Which means that the bounded procedure for searching models of formulae in $\QL^-$ could be used to search for counterexamples of formulae in $\QL$.
% 
Notice that \qSat can be easily extended to return the run that satisfies the formula, if there is one.
Such run can be used to identify the source of QoS formula violations when \qSat is used as a counterexample-finding procedure.
% by considering that non $\grecop$-free g-choreographies can be analysed by:
% \begin{enumerate}[label = \arabic*)] 
% \item translating the formula $\gqosprop$, to be checked for validity,
%   in a way that each iterative g-choreography $\grec[]$ in $\gqosprop$
%   is replaced with $\aG^{(n)}$ for a natural number $n$; for example,
%   $\Psi\ \qluntil[{\grec[][\aG_1]}]\ (\Psi'\
%   \qluntil[{\grec[][\aG_2]}]\ \Psi'')$, gets translated to
%   $\Psi\ \qluntil[{\aG_1^{(2)}}]\ (\Psi'\ \qluntil[{\aG_2^{(5)}}]\
%   \Psi'')$,
% \item expanding the resulting formula according to $\Psi\ \qluntil[{\aG^{(n)}}]\ \Psi' = \bigvee\limits_{i = 0}^{n} \Psi\ \qluntil[{\aG^i}]\ \Psi'$, where $\aG^0 = \aG$ and $\aG^{i+1} = \aG\ ;\ \aG^i$, yielding a formula $\hat \gqosprop$,
% \item checking whether $\neg\hat\gqosprop$ is satisfiable or not.
% \end{enumerate}
% If $\neg\hat\gqosprop$ is satisfiable, then $\hat\gqosprop$ is not valid, which means $\gqosprop$ is not valid either. The reason  is that as any legal run of $\hat\gqosprop$ is a legal run of $\gqosprop$ and, if there is one that does not satisfy $\hat\gqosprop$, it will not satisfy $\gqosprop$.
% On the other hand, if $\neg\hat\gqosprop$ is not satisfiable, $\hat\gqosprop$ is valid. But this does not mean that $\gqosprop$ is valid, because  more unfoldings could be necessary to find a counterexample.

% \begin{theorem}[Decidability of $\QL$]
%   \label{thm:decidability}
%   Given a QoS-extended communicating system $\aCS$ and a QoS formula $\gqosprop \in \QL$, the satisfiability of $\gqosprop$ in $\aCS$ is decidable.
% \end{theorem}

% Given $\gqosprop \in \QL^-$ and a communicating system $\aCS$
% \textsc{qSat}$(\gqosprop, \aCS, \aConf_0)$ returns \textsc{true} iff
%  $\gqosprop$ is satisfiable in $\aCS$, where $\aConf_0$ is the
% initial configuration of $\aCS$.

% Basically, \qModels\ searches the LTS of $S$ for a run extending $\pi$
% and satisfying the formula $\gqosprop$.
% %
% If $\gqosprop$ is a QoS formula (\cref{ln:smt}), \qModels\ invokes a
% satisfaction modulo theories solver~\cite{demoura:cacm-54_9}
% implementing a decision procedure for RCFs; in a prototype
% implementation we used Z3~\cite{demoura:tacas08}.
% %
% \cref{ln:or,ln:and} respectively recur to disjunction and conjunction.
% %
% \cref{ln:quntil} handles modalities by relying on the procedure \qUntil. 
% A call to \qUntil{$\gqosprop_1, \aG, \gqosprop_2,\aCS,\pi_0, \pi_1$} 
% returns \textbf{true} if and only if 
% $$
% \exists \pi^\star \in \Delta^\infty_{\aCS} \text{ such that } \pi_0\pi_1 \in \mathit{prf}(\pi^\star)
%  \text{ and } \conf{\pi^\star, \pi_0} \models \gqosprop\ \qluntil\ \gqosprop'
% $$
% This means that $\gqosprop\ \qluntil\ \gqosprop'$ holds for the run $\pi_0$.
% But it also entails that the continuation of $\pi_0$ (namely $\pi''$) that satisfies $\rlang[\pi''] \in \rlang[\aG]$
% and whose existance is guaranteed by the semantics of the until operator must be an extension 
% of $\pi_1$. Thus, this last parameter $\pi_1$ serves the purpose of remembering the partial continuation
% of the run $\pi_0$ that has been made in search of a satisfying one. 
% \cref{ln:quntil-psi'} deals with the case in which the search finishes 
% with a positive answer after checking if the conditions imposed by the semantics 
% of the until operator hold for $\pi_1$. 
% Otherwise, \cref{ln:quntil-psi,ln:quntil-foreach,ln:quntil-recursion} continue the search.
% \cref{ln:quntil-psi} checks that $\gqosprop$ holds for the partial extension $\pi_0\pi_1$ 
% as imposed by the semantics for every partial extension. \cref{ln:quntil-foreach} goes trought 
% all possible transitions for extending $\pi_1$ and only considers those that are compatible 
% with $\rlang[\aG]$. Finally, \cref{ln:quntil-recursion} continues the search in those extensions
% by recursively calling to \qUntil. If at least one of this extensions finds a positive answer
% the algorithm returns \textbf{true}, otherwise it returns \textbf{false}.
% % between
% % $\gqosprop_1\ \qluntil[]\ \gqosprop_2$ and
% % $\gqosprop_2 \lor \left(\gqosprop_1 \land \bigcirc\left(\gqosprop_1\ \qluntil[]\
% % 	 \gqosprop_2\right)\right)$,
% % %
% % where $\bigcirc$ is the \emph{next} operator.
% % %
% % Accordingly, \qModels\ uses the functional
% % $F (X, Y) = Y \lor \left(X \land \bigcirc\left(F (X, Y)\right)\right)$
% % to resolve modalities by computing the minimal fix-point of
% % $F (\gqosprop_1,\gqosprop_2)$.
% %
% Notably, the recursive call is performed only if the trace of
% $\pi \cdot \aConf \TRANSS{\al} \aConf'$ is in $\rlang[\aG]$.
% %
% This guarantees termination since $\rlang[\aG]$ is finite, both in its cardinal and in the length of its elements.
% %
% % As all possible extensions of $\pi$ are evaluated at \cref{5,6},
% % whenever no extension is feasible (by finiteness of
% % $\rlang[\aG]$), the iteration concludes with the verdict that the
% % property is not satisfied.
% %

% Like for other model-checking procedures, \qModels\ can be used to
% check validity of  $\QL^-$ formulae.
% % 
% This is done by checking the satisfiability of the negated formula.
% Based on \qModels, we define a bounded model-checking approach for $\QL$
% by considering that non $\star$-free g-choreographies can be analysed by:
% \begin{enumerate}[label = \arabic*)] 
% \item translating the formula $\gqosprop$, to be checked for validity,
%   in a way that each iterative g-choreography $\grec[]$ in $\gqosprop$
%   is replaced with $\aG^{(n)}$ for a natural number $n$; for example,
%   $\Psi\ \qluntil[{\grec[][\aG_1]}]\ (\Psi'\
%   \qluntil[{\grec[][\aG_2]}]\ \Psi'')$, gets translated to
%   $\Psi\ \qluntil[{\aG_1^{(2)}}]\ (\Psi'\ \qluntil[{\aG_2^{(5)}}]\
%   \Psi'')$,
% \item expanding the resulting formula according to $\Psi\ \qluntil[{\aG^{(n)}}]\ \Psi' = \bigvee\limits_{i = 0}^{n} \Psi\ \qluntil[{\aG^i}]\ \Psi'$, where $\aG^0 = \aG$ and $\aG^{i+1} = \aG\ ;\ \aG^i$, yielding a formula $\hat \gqosprop$,
% \item checking whether $\neg\hat\gqosprop$ is satisfiable or not.
% \end{enumerate}
% If $\neg\hat\gqosprop$ is satisfiable, then $\hat\gqosprop$ is not valid, which means $\gqosprop$ is not valid either. The reason  is that as any legal run of $\hat\gqosprop$ is a legal run of $\gqosprop$ and, if there is one that does not satisfy $\hat\gqosprop$, it will not satisfy $\gqosprop$.
% On the other hand, if $\neg\hat\gqosprop$ is not satisfiable, $\hat\gqosprop$ is valid. But this does not mean that $\gqosprop$ is valid, because  more unfoldings could be necessary to find a counterexample.

% \paragraph{A note on complexity}
% %Let $\mid X \mid$ denote the cardinality of a set $X$.
% %
% Given a communication system $\aCS$ and a formula $\gqosprop$ to be
% checked, the complexity of \qModels depends on the complexity of
% $\texttt{SMT}(\_)$ and the check for membership in the language of a
% g-choreography.
% %

% The time complexity of \qModels\ in the worst case scenario is
% \begin{align*}
% O( 2^k (d C_{\mathfrak{m}_\gqosprop} +  C_{\text{SMT}_\Phi} ) )
%   \qqand[where]
% \end{align*}

% \begin{itemize}
% \item $k$ is the number of disjunctions in $\gqosprop$,
% \item $d$ is the cardinality of the set of runs of length at most $n$ of $\aCS$, 
% where $n$ is the maximum length of a trace in a language of a
% g-choreographies in $\gqosprop$,
% % \item $\ell$ is the maximal size of the languages of g-choreographies
% %   in $\gqosprop$ (we assume that such languages are pre-computed as a
% %   data structure that provides a membership operation in logarithmic time
% %   in the size of the languages).
% \item $C_{\mathfrak{m}_\gqosprop}$ is an upper bound for
% checking membership in the laguages of g-choreographies
% in $\gqosprop$, and
% \item $C_{\text{SMT}_\Phi}$ is an upper bound for the cost of all of the
%   SMT-solving of the first-order theories resulting from aggregating
%   the QoS specification associated to the states along the traces;
%   notice that this includes also the cost of aggregating QoS
%   attributes with $\aggfn(\_)$.
% \end{itemize}

% The rationale is that every prefix of a trace is checked for
% membership to the language of the g-choreography when its potential
% extension is considered.
% %
% % Also, at that specific point, two recursive check are performed, the
% % one in \cref{4} (considered to fail in the worst case scenario) and
% % the one in the first part of \cref{6}. 
% Then, the $2^k$ factor appears
% because every disjunction forces the algorithm to check both
% subformulae over the whole set of traces starting from the point in
% which the formula appears.

% % A different, more involved, implementation might explore building the
% % languages of the g-choreographies on the fly, instead of pre-computing
% % them. Such an strategy would eliminate $O(C_{\rlang[\aG]})$
% % operations, and the $log(|\rlang[\aG]|)$ multiplicative factor
% % appearing in the ``until'' case due to membership test.


% % Next, in \cref{ex:exec} we show the performance of \cref{alg:check} when it is applied to some of the examples we shown in previous sections,

% % \begin{example}[Execution of the analysis algorithm]
% % \label{ex:exec}
% % \cnote{Choose a property with $\star$ and analyse the bounded version for different bound making explicit number of traces and average/minimum/maximum length. Ideally we should exhibit a property for which there is a counterexample and it is found, a property for which there is a counterexample but it is not found up-to the bounds and a property that does not have a counterexample independently of the chosen bounds.}
% %   \finex
% % \end{example}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> artefact.tex <==
\subsection{Formats of  input files}
\label{sec:input-formats}
We now describe the format of the input files of \thetool through the
simple example shown in \cref{ex:simple-cfsm-qos}.
%
The content of the \texttt{.qosfsa} file describing the system is
shown below.

\begin{wrapfigure}[19]{l}{6cm}
  \lstinputlisting[style=qosfsa]{examples/input-format/sys.qosfsa}
\end{wrapfigure}
 
The text inside the \texttt{fsa} block (lines 2--18) is \chorgram's textual
representation for CFSMs (\texttt{.fsa} files).
% 
Lines 4--7 and 13--16 correspond to the transitions of $\ptp[A]$ and
$\ptp[B]$ respectively.
%
Each transition is represented by a line of the form \texttt{src p act
  msg tgt}, where \texttt{src} and \texttt{tgt} are the source and
target states, \texttt{p} is the index of the partner machine in the system
(\texttt{0} for $\ptp[A]$ and \texttt{1} for $\ptp[B]$),
\texttt{act} is the input (\texttt{?}) or output (\texttt{!})
action, and \texttt{msg} is the message.
%
The QoS attributes are given on line 20 as a list of pairs
\texttt{attr:op} where \texttt{attr} is the name of the attribute and
\texttt{op} is its aggregation operator.
%
The aggregation operator symbol has to be a valid SMT-LIB binary
operator.
%
Lines 21--25 specify the QoS specifications associated to states of
the machines, separated by a comma.
Each one follows the syntax \texttt{name@state : constraint} where
\texttt{name} is the name of the CFSM, \texttt{state} is the identifier
of the state, and \texttt{constraint} is a valid SMT-LIB term where
the only allowed free variables are the names of the QoS attributes.
States that do not appear in the list of QoS specifications do not
have any QoS constraint associated to them (hence the values for their
QoS attributes will not be considered during the analysis).
%
Finally, line 26 specifies the set of final states of each machine.
For each participant we have \texttt{ptp : [states]}, where
\texttt{ptp} is the name of the machine and \texttt{states} is a
comma-separated list of identifiers of the final states of the
machine.

Let $\aG = \gint[][A][x][B]; \gint[][B][y][A]; \gint[][A][z2][B]$ and
suppose we are interested in verifying if the formula
$\possib{\aG}\ (2 \leq \mathit{cost} \leq 3)$ holds in the system
above.
%
\begin{wrapfigure}[6]{l}{5.5cm}
  \vspace{-5pt}
    \lstinputlisting[style=ql]{examples/input-format/prop.ql}
\end{wrapfigure}
%
The textual representation of this formula (file \texttt{.ql}) is shown to the side.
%
The index of the \squo{until} operator is represented on lines 3--5
using \chorgram's g-choreography syntax.
%
The keyword \texttt{qos} on line 7 denotes a QoS constraint atomic
formula, which is specified as a valid SMT-LIB term where the only
allowed free variables are the names of the QoS attributes.
% 

\subsection{Using \thetool}
%%% As we've seen, \thetool requires users to provide a textual description of the QoS-extended communication system they intend to analyze.
%%% The source of this description varies depending on the specific context in which \thetool is employed. In the context of system design, the process typically starts with the designer writing a global view of the system, followed by an automated derivation of CFSMs for the system's participants. Subsequently, the designer proceeds to define QoS specifications for specific states within these machines, as well as specifying its sets of final states. These QoS specifications, together with the communicating aspects of the CFSMs, would act as requirements for the implementation of the system. Any implementation that satisfies these requirements is guaranteed to fulfill any $\QL$ properties that can be verified by \thetool on the QoS-extended communication system.
%%% Conversely, when analyzing an existing system, the user's process begins with the extraction of CFSMs from the existing code. There are existing tools available for this task, tailored to various programming languages \cite{imai:tacas22,imai:places10}. Following this, the user is required to write QoS specifications by examining the implementation. In cases where a service utilizes an external service, these step may also entail consulting the SLA of such service.
As seen, \thetool requires the description of the QoS-extended
communication system.
%
This boils down to assigning a QoS specification to the states of the
communicating machines in the system.
%
It is worth remarking that these machines do not need to be specified
by hand; in fact, one can exploit the \emph{projection} operation of
\chorgram to automatically generate the qCFSMs out of QoS-extended g-choreographies
(\texttt{.qosgc} files introduced earlier),
which are the starting point of top-down choreographic design.
%
This is a main reason for leveraging g-choreographies as
they lift the burden of manually specify local models. 
%
% Thus %%% This allows designers to
% designers can attain qCFSMs by assigning QoS specifications
% to the (relevant) states of projected CFSMs and specifying their final
% states.
%
Alternatively, when analysing existing systems, CFSMs can be
automatically extracted from code.
%
In fact, there exist tools available for this task, tailored to
various programming languages~\cite{imai:tacas22,imai:places10,chorErl}.
%
If the system being analysed was built by
composing existing services, QoS specifications can be extracted from
the SLAs of those services.
% The tool provides a means to verify QoS properties of the composition.

Once the model of the system and the property are specified, the user can invoke \thetool through its Command Line Interface as follows:
%
\begin{center}
\begin{minipage}{.8\linewidth}
\begin{lstlisting}[style=ql, basicstyle=\ttfamily\footnotesize, numbers=none]
 mocheqos <cmd> <qcfsms> <prop> <k> [options]
\end{lstlisting}
\end{minipage}
\qqand[where]
\end{center}
\begin{itemize}
\item \texttt{<cmd>} is the (name of the) operation to apply; it can
  be either \texttt{satisfiability} or \texttt{validity}
   for checking the satisfiability or validity of the property
  \texttt{prop} on the communicating system \texttt{qcfsms};
  in the case of \texttt{validity}, \thetool will negate 
  \texttt{prop} and search for a counterexample,
\item \texttt{<qcfsms>} is the path to a \texttt{.qosfsa} file containing a textual description of the QoS-extended system at hand,
\item \texttt{<prop>} is the path to a \texttt{.ql} file containing a textual description of the $\QL$ formula,
\item \texttt{<k>} specifies the bound on the length of the runs to be considered, and
\item \texttt{[options]} specifies optional requests to \thetool:
\begin{itemize}
  \item \texttt{--unfoldings <u>} specifies the maximum number of
    unfolding of the $\grecop$ operators in the g-choreographies in
    \texttt{<prop>} (\texttt{u} defaults to \texttt{k}.), 
  \item \texttt{--show-model} prints a run that satisfies the property, if any, and
  \item \texttt{--verbose} executes the analysis in verbose mode, which prints the current length of runs being considered 
  and the total number of runs with such length.
\end{itemize}
\end{itemize}
Additionally, the flag \texttt{--help} will print a help message.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> aux.tex <==
%!TEX root = ./main.tex

\begin{definition}[Algebraic operators]\label{def:algop}
  An operator is said to be algebraic if it can be defined by a set of
  first order formula over the signature of the real closed
  fields. Alternatively, we can say that an algebraic operator is one
  that can be defined by algebraic equations, namely by using
  constants symbols, the basic arithmetic operators of the algebra
  $\_+\_$ and $\_ \cdot \_ $ and their opposites $\_-\_$, $\_/\_$,
  and their natural extension $\_^\_$ (exponentiation) and
  $\sqrt[\_]{\_}$ (root). See \cite[\S11.5]{hardy38} for an extensive
  discussion on algebraic equations and the mathematical properties of
  algebraic numbers.
\end{definition}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> auxrcf.tex <==
%!TEX root = ./main.tex

\begin{definition}[Ordered Field -- \cite{birkhoff65}(Sec.~2.1)]\label{def:ofield} 
Let $\Sigma_{\mathrm{field}} = \conf{\{0, 1\},\{+, \cdot\},\{=\}}$ and $\Gamma_{\mathrm{field}}$ the set containing the following formulae:
  $$
  \begin{array}{ll}
\text{(associativity)} & (\forall x, y, z)( x \cdot (y \cdot z) = (x \cdot y) \cdot z \land x + (y + z) = (x + y) + z)\\
\text{(commutativity)} & (\forall x, y)(x \cdot y = y \cdot x \land x + y = y + x)\\
\text{(identities)} & (\forall x)(x \cdot 1 = x \land x + 0 = x)\\
\text{(distributivity)} & (\forall x, y)(\forall z)x \cdot (y + z) = (x \cdot y) + (x \cdot z)\\
\text{($\cdot$ inverses)} & (\forall x)(x =  0 \lor ((\exists y) x \cdot y = 1))\\
\text{($+$ inverses)} & (\forall x)((\exists y) x + y = 0)
  \end{array}
  $$
Then, any model of the (first order) theory presentation $\conf{\Sigma_{\mathrm{field}}, \Gamma_{\mathrm{field}}}$ is said to be a \emph{field}.
%
An \emph{ordered field} is a field with a strict totally ordered
\footnote{Let $S$ be a set then $\leq \subseteq S \times S$ is a
  \emph{total order} if it satisfy the following conditions:
    \begin{inparaenum}[\itshape a\upshape)]
    \item Reflexivity: for all $a \in S$, $a = a$,
    \item Antisymmetry: for all $a, b, c \in S$, if $a \leq b$ and $b \leq a$ then $a = b$,
    \item Transitivity:  for all $a, b, c \in S$, if $a \leq b$ and $b \leq c$ then $a \leq c$, and
    \item Totality: for all $a, b \in S$, $a \leq b$ or $b \leq a$.
    \end{inparaenum}
Additionally, given $\leq \subseteq S \times S$ a total order, its associated \emph{strict total order} $< \subseteq S \times S$ is be defined by one of the following equivalent conditions:
    \begin{inparaenum}[\itshape a\upshape)]
    \item Reflexive reduction: for all $a, b \in S$, if $a \leq b$ and $\neg a = b$, then $a < b$, or
    \item $<$ is the complement of the converse of $\leq$: for all $a, b \in S$, if $\neg a \leq b$, then $a < b$.
    \end{inparaenum}
  } 
carrier set.
\end{definition}

Real-closed fields are ordered fields whose non-empty subsets all have a supremum.

\begin{definition}[Real-closed field -- \cite{birkhoff65}(Sec.~4.3)]\label{def:RCF}
  Given an ordered field with carrier $S$, its order
  $\leq \subseteq S \times S$ is \emph{Dedekind-complete} if every
  non-empty subset $S' \subseteq S$ with an upper bound in $S$ has a
  least upper bound (also called supremum) in $S$.
 
  Whenever $\leq$ is Dedekind-complete, the ordered field is said to
  be the \emph{real-closed field} (or a \emph{Dedekind-complete
    ordered field}).
\end{definition}

Intuitively, in Dedekind's own words, completeness implies that there
are not any \quo{gaps} in the real line, forcing the set to be
continuous.

 \begin{theorem}[Isomorphism of Real-closed fields \cite{erdos:am-3_61}(Thm.~2.1)]
   Under the continuum hypothesis, all hyper-real fields of power
   $\aleph_1$ are isomorphic.
 \end{theorem}

 \begin{corollary}
 \label{isomorphism}
 Given any two Dedekind-complete ordered fields with carrier sets $S$
 and $S'$ respectively, there exists a unique order-preserving field
 isomorphism from $S$ to $S'$.
 \end{corollary}

 In \cite{tarski:RM-109}, Tarski introduced what he called \emph{the system of elementary algebra}, his formalisation of the real numbers, as an ordered field (see \cite[Note~9]{tarski:RM-109}) also satisfying:
 \begin{inparaenum}[\itshape a\upshape)]
 \item an axiom stating that every positive number has a square root, and
 \item an axiom scheme stating that every polynomial of odd degree has, at least, one real root,
 \end{inparaenum}
 resulting in a first order theory that can be proved to be a Dedekind-complete ordered field \cite[Note~15]{tarski:RM-109}.
 \footnote{The proof of is obtained by first defining the topological completion of an ordered field $\mathit{F}$ by Dedekind cuts (denoted $\mathit{Dc}(\mathit{F})$) and then proving that, on the one hand:
 \begin{inparaenum}[\itshape a\upshape)]
 \item any polinomial of odd degree in an ordered field $\mathit{F}$, has a root in the topological completion $\mathit{Dc}(\mathit{F})$, and
 \item any element greater that $0$ in an ordered field $\mathit{F}$, has a square root in the topological completion $\mathit{Dc}(\mathit{F})$;
 \end{inparaenum}
 and, on the other hand, recalling that the topological completion $\mathit{Dc}(\mathit{F})$ of an ordered field $\mathit{F}$ satisfies the axioms of the system of elementary algebra.}.
 
 By \cref{isomorphism}, Tarski's system of elementary algebra is isomorphic to the real-closed field (see \cref{def:RCF}). Furthermore, Tarski proves that his system admits quantifier elimination \cite[Coro.~32]{tarski:RM-109} and, consequently, the existence of a decision procedure \cite[Thm.~37]{tarski:RM-109}.
 Tarski's decision procedure is of non-elementary complexity, meaning that given a problem of size $n$, it's complexity is not bound by any function of the form ${{{{2^2}^\cdot}^\cdot}^\cdot}^n$. In \cite{monk+:manuscript74}, Monk provided an elementary complexity algorithm quantifier elimination. In \cite[Corollary to Thm.~1]{davenport:jsc-5_1} Davenport and Heintz proved that quantifier elimination for real-closed field is doubly exponential in the size of the problem. Algorithms of such a complexity were provided by Collins in \cite{collins:atfl75}, and Monk in \cite{monk+:phdthesis}, independently. Later, in \cite{ben-or:jcss-32_2}, Ben-Or et. al proposed a different algorithm running in exponential space or parallel exponential time in the size of the problem.\\


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> chor.tex <==
%!TEX root = ./main.tex
%
We use \emph{global choreographies}~\cite{tuosto:jlamp-95} to specify
the global view of communicating systems whose local view are rendered
as \emph{communicating finite state machines}~\cite{brand:jacm-30_2}.

Hereafter, we fix a set $\PSet$ of \emph{participants} and a set
$\msgset$ of (types of) \emph{messages} such that
$\PSet \cap \msgset = \emptyset$.
%
We start by surveying the definition of g-choreographies.

\begin{definition}[Global choreographies~\cite{tuosto:jlamp-95}]\label{def:g-choreography}
  A \emph{global choreography over $\PSet$ and $\msgset$}
  (\emph{g-choreography} for short) is a term $\aG$ that can be
  derived in
  \begin{align*}
	 \aG \bnfdef \gempty \bnfmid \gint[] \bnfmid \gseq[] \bnfmid \gpar[]
	 \bnfmid \gcho[] \bnfmid \grec
  \end{align*}
  where $\p, \q \in \PSet$, $\p \neq \q$ and $\msg \in \msgset$.
\end{definition}
%
Intuitively, a g-choreography specifies the communication protocol of
participants.
%
The basic g-choreography is the empty one $\gempty$, which specifies
that no communications should happen.
%
An \emph{interaction} $\gint[]$ specifies that participants $\p$ and
$\q$ (are expected to) exchange a message of type $\msg$;
%
  it is worth remarking that we assume asynchronous communication
  where the sender $\p$ does not wait for $\q$ to consume $\msg$
  to continue its execution.
  %
%
Moreover, g-choreographies can be composed sequentially ($\gseq[]$),
in parallel ($\gpar[]$), and in non-deterministic choices
($\gcho[]$); we assume that $\gempty$ is the neutral element
  of $\gseq[][\_][\_]$, $\gpar[][\_][\_]$, and $\gcho[][\_][\_]$.
  Note that, due to asynchrony in the communication, in a sequential
  composition $\gseq[]$, outputs in $\aG'$ can occur before $\aG$ is
  fully executed; for instance, the distributed execution of
  $\gseq[][{\gint[]}][{\gint[][c][m'][b]}]$ allows the output from
  $\ptp[c]$ to happen before the one from $\p$.
  %
%
Finally, a g-choreography may be iterated ($\grec[]$).

\begin{example}[A g-choreography for POP]\label{ex:gpop}
  Our running example can be expressed as the g-choreography
  $\gpop{pop} =
  \gcho[][{\gseq[][{\gint[][c][helo][s]}][{\gpop{start}}]}][{\gpop{quit}}]$
  where
  \begin{align*}
	 \begin{array}{l@{\quad}l}
		\gpop{start} = 
    \gseq[][
      {\gint[][s][int][c]}
      ][
        {\gseq[][
          {\grec[][({\gcho[][\gpop{read}][{\gseq[][\gpop{read}][\gpop{retr}]}]})]}
          ][
            {\gpop{quit}}
            ]
        }
        ]
		& \gpop{read} = \gseq[][{\gint[][c][read][s]}][{\gint[][s][size][c]}]
		\\
		\gpop{retr} = \gseq[][{\gint[][c][retr][s]}][{\gint[][s][msg][c];\gint[][c][ack][s]}]
		& \gpop{quit} = \gseq[][{\gint[][c][quit][s]}][{\gint[][s][bye][c]}]
  \end{array}
\end{align*}
($\gseq[][\_][\_]$ takes precedence over $\gcho[][\_][\_]$).
%
% We remark that messages specify just the type of a message and not their payload.
% 
\finex
\end{example}

The participants of a communicating system interact through
\emph{channels} borrowed from the set
$\chset = \set{(\p, \q) \in \PSet \times \PSet \sst \p \neq \q}$.
%
A channel $(\p,\q) \in \chset$ (written $\achan$ for short) allows
$\p$ to asynchronously send messages to $\q$ through an unbounded FIFO
buffer associated to $\achan$.
The set of \emph{communication actions} is
$\lset = \lset^!  \cup \lset^?$ where
$\lset^! = \{ \aout \sst \achan \in \chset \text{ and } \msg \in
\msgset\}$ and
$\lset^? = \{ \ain \sst \achan \in \chset \text{ and } \msg \in
\msgset\}$ are respectively the set of \emph{output} and \emph{input}
actions.
%
% For the purpose of this work we are interested in identifying
The \emph{language} $\rlang[\aG]$ of a g-choreography $\aG$ %. This
is essentially the set of all possible sequences in $\lset$
% of communication actions that are
compatible with the causal relation induced by $\aG$.
% and will be noted as $\rlang[\aG]$.
Since $\rlang[\aG]$ is prefix-closed, we write $\hat{\rlang}[\aG]$
for the set of sequences in $\rlang[\aG]$ that are not proper prefixes
of any other sequence in $\rlang[\aG]$.
The technical definition of $\rlang[\aG]$, immaterial here,
% requires a formal semantics for the g-choreography, we 
% present in \cref{sec:sem} a definition that rely on the pomset semantics of g-choreographies that
can be found in~\cite{tuosto:jlamp-95}. %~\cite{pratt:ijpp-15_1,tuosto:jlamp-95}.
% 
We will adapt CFSM~\cite{brand:jacm-30_2} to model the QoS-aware \emph{local
  view} of a system.

\begin{definition}[Communicating systems~\cite{brand:jacm-30_2}]\label{def:cfsm}
  A \emph{communicating finite-state machine} (\emph{CFSM})
  is a finite transition system $\aCM = (\aQ,\aQzero,\aTrs)$ where
  \begin{itemize}
  \item $\aQ$ is a finite set of {\em states} with $\aQzero \in \aQ$
	 the \emph{initial} state, and
  \item $\aTrs\ \subseteq \ \aQ \times \lset \times \aQ$; we write
	 $q \trans{\al} {q'}$ for $(q,\al,q') \in \aTrs$.
  \end{itemize}
  %
  For $\aout \in \lset$ (resp.  $\ain \in \lset$), let
  $\subject[\aout] = \p$ (resp.  $\subject[\ain] = \q$).
  %
  Given $\p \in \PSet$, $\aCM$ is \emph{$\p$-local} if
  $\subject[\al] = \p$ for each $q \trans{\al} {q'}$.
  %
  A \emph{(communicating) system} is a map
  $\aCS = (\aCM_{\ptp})_{\ptp \in \ptpset}$ assigning a $\p$-local
  CFSM $\aCM_{\ptp}$ to each $\ptp \in \ptpset$.
\end{definition}

\begin{example}[Communicating system for POP]\label{ex:pop}
    The following CFSM exhibits a behaviour of a POP client
    compatible with the protocol in
    \cref{ex:gpop} because its executions yield a subset of 
    the client's execution specified there.
% 
{\small  \begin{align*}
%  \includegraphics[width=0.8\textwidth,valign=c]{ex-pop-client.pdf}
   \begin{tikzpicture}[node distance=1cm and 1.3cm, every node/.style={scale=1,transform shape}]
	 \node (d) at (0,0) {};
	 \node[cnode,right= .3cm of d] (0) {};
	 \foreach \s/\t in {0/1,1/2,2/3,3/4,4/5,5/6} {
		\node (\t) [cnode, right = of \s] {};
	 }
	 \foreach \s/\l/\t in {0/\aout[c][s][helo]/1,1/\ain[s][c][int]/2,2/\aout[c][s][read]/3,3/\ain[s][c][size]/4,4/\aout[c][s][retr]/5,5/\ain[s][c][msg]/6} {
		\path[line,sloped] (\s) edge node[below]{$\l$} (\t);
	 }
	 \node[cnode,above = of 0] (7) {};
	 \node[cnode,right = of 7] (8) {};
	 %
	 \path[line] (d) -- (0);
	 \path[line] (6) edge[bend left=-35] node[below]{$\aout[c][s][ack]$} (2);
	 \path[line] (0) edge node[left]{$\aout[c][s][quit]$} (7);
	 \path[line] (2) edge node[left]{$\aout[c][s][quit]$} (7);
	 \path[line] (4) edge[sloped] node[above]{$\aout[c][s][quit]$} (7);
	 \path[line] (7) edge node[above]{$\ain[s][c][bye]$} (8);
  \end{tikzpicture}
  \end{align*}
}  %
  For a POP server, being a two-party protocol, we can use a dual CFSM obtained by replacing
  send actions with corresponding receive actions and
  vice versa.
  %
  \finex
\end{example}
%
% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.8\textwidth,valign=c]{ex-pop-client.pdf}
% \caption{CFSM of a \textit{Client} in the simplified POP protocol.}
% \label{fig:ex-pop}
% \end{figure}

The asynchronous communication between participants is formalised by a labelled transition system (LTS) tracking the
(local) state of each CFSM and the content of each buffer (i.e. communication channel) in the
system.
%
A \emph{configuration} of a communicating system $\aCS$ is a pair
$\aConf = \csconf q \abuffer$ where $\vec q$ and $\vec \abuffer$
respectively map participants to states and channels to sequences of
messages; state $\vec q(\p)$ keeps track of the state of the machine
$\aCM_{\p}$ and buffer $\abuffer(\achan)$ yields the messages
sent from $\p$ to $\p[b]$ and not yet consumed.
%
The \emph{initial} configuration $\aConf_0$ is the one where, for all
$\p \in \ptpset$, $\vec q(\p)$ is the initial state of the
corresponding CFSM and $\abuffer(\achan)$ is the empty sequence for
all $\achan \in \chanset$.

A configuration $\aConf'= \csconf {q'} {\abuffer'} $ is {\em
  reachable} from another configuration
$\aConf = \csconf {q} {\abuffer}$ by \emph{firing a transition $\al$},
written $\aConf \TRANSS{\al} \aConf'$, if there is a message
$\msg \in \msgset$ such that either (1) or (2) below holds:
\begin{center}
  \begin{tabular}{l@{\hspace{.45cm}}r}
    \begin{minipage}{.47\linewidth}\small
      1.  $\al = \aout[@][@][@]$ with
		$\vec q(\p) \trans[\p]{\al} {q'}$ and
        \begin{itemize}
        \item[a.] $\vec q' = \vec q[\p \mapsto q']$
        \item[b.] $\abuffer' = \abuffer[\achan \mapsto \abuffer(\achan).\msg]$
        \end{itemize}
    \end{minipage}
    &
    \begin{minipage}{.47\linewidth}\small
      2.
        $\al = \ain[@][@][@]$ with $\vec q(\q) \trans[\q]{\al} {q'}$
        and 
        \begin{itemize}
        \item[a.] $\vec q' = \vec q[\q \mapsto q']$ and
        \item[b.] $\abuffer = \abuffer'[\achan \mapsto \msg.\abuffer'(\achan)]$.
        \end{itemize}
    \end{minipage}
  \end{tabular}
\end{center}
%
Condition (1) puts $\msg$ on channel $\ptp\ptp[B]$, while (2) gets
$\msg$ from channel $\ptp\ptp[B]$.
%
In both cases, any machine or buffer not involved in the transition
is left unchanged in the new configuration $\aConf'$.
\begin{example}[Semantics of CFSMs]
  For the run $\pi$ of the communicating system in \eqref{eq:idea}
  (cf. \cref{sec:intro}) we have, for $i \in \{0,1,2\}$,
  $\aConf_i = \csconf{q_i}{\abuffer_i}$, where
  $\vec{q_0} = \{\p \mapsto \aQzero, \q \mapsto \aQzero'\}$,
  $\abuffer_0 = \{\achan \mapsto \epsilon,
  \achan[b][a] \mapsto \epsilon\}$,
  $\vec{q_1} = \{\p \mapsto q_1, \q \mapsto \aQzero'\}$,
  $\abuffer_1 = \{\achan \mapsto \msg, \achan[b][a] \mapsto
  \epsilon\}$, and $\vec{q_2} = \{\p \mapsto q_1, \q \mapsto q_1'\}$,
  $\abuffer_2 = \abuffer_0$.
  %
  \finex
\end{example}
Let $\aCS$ be a communicating system.
%
A sequence $\pi = (\aConf_i,\al_i,\aConf_{i+1})_{i \in I}$ where
$I$ is an initial segment of natural numbers (i.e., $i-1 \in I$ for
each $0 < i \in I$) is a run of $\aCS$ if
$\aConf_i \TRANSS{\al_i} \aConf_{i+1}$ is a transition of $\aCS$ for
all $ i \in I$.
%
The set of runs of $\aCS$ is denoted as $\Delta^\infty_{\aCS}$
and the set of runs of length $k$ is denoted as $\Delta^k_{\aCS}$.
Note that $\Delta^\infty_{\aCS}$ may contain runs of infinite length, 
the set of finite runs of $\aCS$ is the union of all $\Delta^k_{\aCS}$ 
and will be denoted as $\Delta_{\aCS}$.
%
Given a run $\pi$,
%$ = (\aConf_i,\al_i,\aConf_{i+1})_{i \in I}$
 we define
$\rlang[\pi]$ to be the sequence of labels $(\al_i)_{i \in I}$.
%
The \emph{language} of $\aCS$ is the set
$\rlang[\aCS] = \{\rlang[\pi] \sst \pi \in
\Delta^\infty_{\aCS}\}$.
%
Finally, $\mathit{prf}: \Delta^\infty_{\aCS} \to 2^{\Delta_{\aCS}}$
maps each run $\pi \in \Delta^\infty_{\aCS}$ to its set of finite
prefixes.
%
As usual, for all $\pi \in \Delta^\infty_{\aCS}$,
the
empty prefix
$\epsilon$ belongs to $\mathit{prf} (\pi)$.
%
For convenience, we will occasionally write
$ \aConf_0 \TRANSS{\al_0} \aConf_1\ \ldots\
 %\aConf_i \TRANSS{\al_i} \aConf_{i+1}\ \ldots\ 
\aConf_n \TRANSS{\al_n} \aConf_{n+1}$ for finite sequences.
% \enote{why do we define compliance? It does not seem to be used}\cnote{It is used to define satisfaction of PDLTL formulae by a communicating system because Until operators are indexed by global graphs.}
% Now, with these formal tools, one would like to tell if a set of local
% artifacts behave accordingly to the interactions prescribed by the
% correspondent global view. Since we are only modeling message-passing
% behaviour what we would like to see is that all the possible
% interactions between the set of local artifacts are behaviours allowed
% by the choreography.

% \begin{definition}[Compliance]
%   A communicating system $\aCS = ( \mathit{M}_{\p} )_{\p \in \PSet}$
%   \emph{complies} with a g-choreography $\aG$ if:
%   $\rlang [S] \subseteq \rlang [\aG]$, that
%     is, all runs of the communicating system are licit runs of the
%     choreography.
% \end{definition}
%Informally, the language $\rlang [\aG]$ of a g-choreography $\aG$ is the sequences of words over the alphabet consisting of the communication actions of the events in $\aG$ that preserve the causal relations allowed in the global view. The formal definition can be found in \cite[Sec.~4.3]{tuosto:jlamp-95}. The intuition behind the language $\rlang [S]$ of a communicating system $S$ is similar, the formal definition can also be found in \cite{tuosto:jlamp-95}.\\


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> evaluation.tex <==
%!TEX root = ./main.tex

The performance\footnote{
  %
  For our experiments we used Z3 version 4.10.2 and an 8-cores MacBook
  Pro (Apple M1) with 16GB of memory.
}
%
of \thetool depends on the cost of checking if a
formula $\Phi$ holds on any run of the system $S$ of length at most
\texttt{k}; this cost is dominated by the evaluation of the
\squo{until} sub-formulae\footnote{%
  This requires to query the SMT-LIB to solve QoS constraints; our
  evaluation does not focus on the cost of executing Z3 to solve the
  SMT-LIB queries (which might increase with the complexity of the QoS
  constraints) since Z3 is used as a black-box which we cannot
  control.
  %
}
$\Phi_1 \qluntil \Phi_2$ which depends on the complexity of $\aG$
and of $\Phi_1$ and $\Phi_2$.
%

We borrow a case study from the AWS cloud~\cite{aws:cloud}.
%
The pricing scheme of the AWS Cloud hinges on a specific list of
attributes whic can be classified as
\begin{itemize}
\item cumulative, like storage (provided by the AWS Elastic Block
  Storage service~\cite{aws:ebs}), measured in Gb and paid per
  month of provisioned storage and, computation (provided by the AWS
  Elastic Compute Capacity service~\cite{aws:ec2}) and software execution, both
  paid per hours of compute time, and
\item non-cumulative, like region and fulfillment option, both ranging
  over a finite list of possible values, and impacting on the unitary
  values paid for the cumulative
\end{itemize}
In addition to the parametric pricing scheme mentioned above, the selection of a specific server configuration for deploying the service, being this another non-cumulative attribute, have a direct impact on other quantitative attributes of interest, like, for example, the transfer rate, which, in turn, impact the final price that will be paid in a given month.

In principle, there are two obstacles for interpreting AWS’ SLAs within the contracts in~\cite{lopezpombo:ictac23}. On the one hand, there is a granularity mismatch between AWS’s SLAs (i.e., the pricing scheme) and the more structured view of process presented in our work. While AWS’s SLAs can be considered monolithic, our automata-based language formalizes components as a composition of tasks represented by the nodes, expressing computations and communication interaction represented by the arrows. This way of describing the behavior of participants provide a more fine-grain view of how the service is executed allowing also a compositional understanding of the costs involved in it. On the other hand, while it is very easy to model the price as the result of accumulating the base values per time/storage unit, multiplied by the time/space required, scaled by the transfer rate, it is important to consider that non-cumulative attributes, which determine the base values, are not directly representable in our approach because attributes are always interpreted as real.

For the sake of showing the potential behind our proposal we will take the SLAs available at AWS marketplace and feature a version of it but compatible with the formal language proposed in our work; in addition, we will represent non-cumulative attributes by building a bijection between the discrete choices in the list and natural numbers. Then, the specification of all the possible configuration can be modeled by a collection of formulae with the shape ``$\left( \bigwedge [ \mathit{non\_cummulative\_attr} ] = [ \mathit{natural\_number} ] \right) \implies \left( \bigwedge [ \mathit{attr} ] = [ \mathit{value} ] \right)$'' therefore, choosing a specific configuration for the service pricing scheme from the available ones boils down to assigning a combination of natural numbers to the corresponding non-cumulative attributes determining the configuration. 

%%%%%

Secondly, we will evaluate the technique over communicating systems
automatically extracted from code. In~\cite{imai:tacas22}, Imai et. al. 
presented a library capable of verifying the compatibility of concurrent
message-passing programs.
%
This library features a type inference algorithm that extracts CFSMs
directly from OCaml code.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
 






\subsection{Experiments}
Our experiments were tailored to address the following
  questions on the performance and effectiveness of \thetool:
  \begin{description}
  \item[Loop unfolding] How does performance evolve, in the best
	 and worst case scenarios, as the number of loop unfolding in the
	 g-choreography of the \squo{until} operator increases?
  \item[Nested choices] How does average performance
	 evolve as the number of nested choices in the g-choreography of
	 the \squo{until} operator increases?
  \item[Model extraction] What is the effectiveness in analysing properties of communicating systems automatically extracted from code?
  \end{description}
%
For the scalability evaluation, we generate synthetic properties
following the pattern $\Phi \equiv \Phi_1 \qluntil \Phi_2$
and varying the size and complexity of $\aG$.
%
Formulas $\Phi_1$ and $\Phi_2$ are created to cover ($i$) the best
case (any run that matches the language of $\aG$ satisfies $\Phi$),
($ii$) the worst case (no run matching the language of $\aG$ satisfies
$\Phi$), and ($iii$) the `average' case (only a single run that matches
the language of $\aG$ satisfies $\Phi$).
% 
For the applicability evaluation, we consider the communicating system
of a case study presented in \cite{imai:tacas22}, which was
automatically extracted from OCaml code. We manually write QoS
specifications for the system, propose $\QL$ formulas to be checked in
the model, and verify them using \thetool.


\subsection{Loop unfolding}
\marginpar{Rewrite everything and explain example}

While, in general, we will resort an example borrowed from~\cite{lopezpombo:ictac23}, in this work we will accommodate the quantitative information to the SLA obtained from AWS marketplace for the services under the modeling criteria discussed above. Figure~\ref{ex:pop-cfsm-qos} shows (part of) the specification of the server participant.\\


we take the running example from \cite{lopezpombo:ictac23} and 


To this purpose, we selected iRedMail, a POP Mail server available at the AWS marketplace \footnote{Documentation available at \url{https://aws.amazon.com/marketplace/pp/prodview-di3vrfwhhpp4k?sr=0-2&ref_=beagle&applicationId=AWSMPContessa}.}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old POP example
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\low{\Gamma_\mathrm{Low}}
\def\db{\Gamma_\mathrm{DB}}
\def\mem{\Gamma_\mathrm{Mem}}
\def\chk{\Gamma_\mathrm{Chk}}
\begin{example}[qCFSMs~\cite{lopezpombo:ictac23}]\label{ex:pop-cfsm-qos}
  The qCFSM $\aCM_{\p[c]}$ below specifies the communication behaviour
  of a POP client \p[c] interacting with a server \p[s]:
  \begin{align*}
	 \aCM_{\p[c]} = &
  \begin{tikzpicture}[node distance=1cm and 1.3cm, every node/.style={scale=1,transform shape}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
	 \node[cnode, initial, initial text={}, label={-95:$\low$}] (0) {};
	 \foreach \s/\l/\t in {0/\low/1,1/\db/2,2/\low/3,3/\db/4,4/\mem/5,5/\chk/6} {
		\node (\t) [cnode, right = of \s, label={$\l$}] {};
	 }
	 \foreach \s/\l/\t in {0/\aout[c][s][helo]/1,1/\ain[s][c][int]/2,2/\aout[c][s][read]/3,3/\ain[s][c][size]/4,4/\aout[c][s][retr]/5,5/\ain[s][c][msg]/6} {
		\path[line,sloped] (\s) edge node[below]{$\l$} (\t);
	 }
	 \node[cnode, above = of 0, label={95:$\low$}] (7) {};
	 \node[cnode, accepting, right = of 7, label={10:$\low$}] (8) {};
	 %
	 \path[line] (6) edge[bend left=-35] node[below]{$\aout[c][s][ack]$} (2);
	 \path[line] (0) edge node[left]{$\aout[c][s][quit]$} (7);
	 \path[line] (2) edge[sloped] node[below,near end]{$\aout[c][s][quit]$} (7);
	 \path[line] (4) edge[sloped] node[above]{$\aout[c][s][quit]$} (7);
	 \path[line] (7) edge node[above]{$\ain[s][c][bye]$} (8);
  \end{tikzpicture}
  \end{align*}
  The only final state of $\aCM_{\p[c]}$ is the doubly-circled one
  and the QoS specifications
  \begin{align*}
    & \low = \{t \leq 0.01, c \leq 0.01, m \leq 0.01\},
	 \\
    & \chk = \{ t \leq 5, c = 0.5, m = 0 \}, \\
		& \mem = \{ 1 \leq t \leq 6, c = 0, m \leq 64 \}, \qand
	 \\
    & \db = \{ t \leq 3 \implies (\exists x)(0.5 \leq x \leq 1 \land c = t \cdot x),
                                            t > 3 \implies c = 10,
                                            m \leq 5 \}
  \end{align*}
  constrain the monetary cost $c$, the execution time $t$, and the
  memory usage $m$ as follows.
  %
  Intuitively, $\low$ specifies that the state performs negligible
  computations, $\chk$ constrain the attributes to check the
  integrity of a message, $\mem$ specifies the allocation of memory for
  a message, and $\db$ to establishing that the monetary cost is fixed
  if a database insertion takes more than three time-units and it is a
  fraction of the execution time, otherwise.
  %  
  \finex
\end{example}

We use a three-party version of the POP protocol introduced in
\cref{ex:pop-cfsm-qos} with an authentication server \p\ (modelled
after the \emph{OAuth} authentication protocol~\cite{rfc6749}). The
participants follow the g-choreography $\aG_{\mathsf{auth}}$ defined as:
\begin{lstlisting}[language=sgc, basicstyle=\footnotesize]
  $\aG_{\mathsf{auth}}$ = $\ \gint[][c][cred][a]$;($\gcho[][{\aG_{\mathsf{token}}}][{\gint[][a][error][c]}]$)
  $\aG_{\mathsf{token}}$ = $\ \gint[][a][token][c]$;$\gint[][c][token][s]$;($\gint[][s][fail][c]$ + $\ \gint[][s][ok][c]$;$\aG_{\mathsf{POP}}$)
\end{lstlisting}
% The authentication server certifies 
% the identity of the client and hands out an authentication token to the
% client. The client then sends the authentication token to the server
% to prove its identity and, if the token is valid, the pop protocol
where $\aG_{\mathsf{POP}}$ is as in \cref{ex:pop-cfsm-qos}. %%% \p[c]$ and $\p[s]$ continue the interaction in $\aG_{\mathsf{retr}}$ with successive retrievals of messages from the mailbox as presented in \cref{ex:pop-cfsm-qos}.
%
	 %
	 The client machine contains 15 states and 17
	 transitions %%% 13 states and 16 transitions,
	 the server machine consists of 12 states 14
	 transitions, %%% the server 10 states and 13 transitions,
	 and the authentication server 4 states and 3 transitions.
	 %
	 The LTS of the whole system consists of 34 states and 38 transitions.
	 %
	 (The CFSMs for \p[c], \p[s], and \p\ as well as the LTS are
	 reported in \cref{appendix:aws}.)
	 %
% 
%%% See \cref{appendix:aws} for a detailed description of
%%% the model used in this case study.  The LTS of the composition of
%%% the three machines contains 33 states and 39 transitions.

While these numbers might not seem particularly high, due to interleaving
\begin{wrapfigure}[13]{r}{6cm}
  \vspace{-9pt}
    \includegraphics[width=0.49\textwidth]{images/evaluation/pop-runs}
    \caption{Size of search space versus \texttt{k}}
    \label{fig:eval:pop-runs}
\end{wrapfigure}
of the transitions
in asynchronous communication, the number of runs of the system grows
exponentially when the number of loop unfoldings in the POP protocol
increases, as shown in \cref{fig:eval:pop-runs}.
%
Moreover, it is worth recalling that CFSMs abstract away from local
computations and focus only on the communication actions. Hence, the
number of states and transitions only reflect the size of the
communication protocol and not necessarily the size of the
implementation.

We attach a simple QoS specification to every state of each machine in
the POP protocol, determining the value of five QoS attributes.
% 
Then, we synthetically generate six families of $\QL$ formulas with the shape $\Phi_1 \qluntil \Phi_2$ where
$\aG = \aG_\mathsf{init};{\aG_\mathsf{msg}}^n$, for $1 \leq n \leq 10$,
where $\aG_\mathsf{init}$ describes the initial interactions before any retrieval\footnote{
     $\aG_{\mathsf{init}} = \ \gint[][c][cred][a];\gint[][a][token][c];\gint[][c][token][s];\gint[][s][ok][c];\gint[][c][helo][s];\gint[][s][int][c]$
 % C -> A : cred; A -> C: token; C -> S: token; S -> C: ok; C -> S: helo; S -> C: int
}
and
$\aG_\mathsf{msg}$ characterises the reading of one message from the mailbox (cf. \cref{ex:gc-pop}).
The first three families of formulas are constructed to be satisfiable while the last three to be unsatisfiable.
The unsatisfiable formulas are constructed by guaranteeing that no run compatible with $\aG$ satisfies $\Phi_2$.
For each formula we execute \thetool with a bound ${\tt k} = 16 + 10n$, which guarantees that the runs of the system that match $\aG$ are reached.
In this way, \texttt{k} ranges between 16 and 116, and the size of the search space for each \texttt{k} is precisely the one shown in \cref{fig:eval:pop-runs}.
In \cref{fig:eval:sat} we plot the time it takes for \thetool to find a model for the three families of satisfiable formulas as a function of $n$. 
The three families differ in how $\Phi_1$ and $\Phi_2$ are defined:
\begin{inparaenum}[(i)]
    \item both as atomic truth values,
    \item $\Phi_1$ as an atomic truth value and $\Phi_2$ is a QoS constraint, or
    \item both as QoS constraints.
\end{inparaenum}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finally, in \cref{fig:eval:unsat} we plot the time it takes for \thetool to report that no model was found for the three families of unsatisfiable formulas as a function of $n$.
The results show that the main source of computational burden, as the number of loop unfoldings increases, is the verification of the QoS constraint in $\Phi_1$, the first operand of the \squo{until} operator. In \cref{fig:eval:sat} and \cref{fig:eval:unsat}, this is manifested by the green line growing significantly faster than the other two lines. The explanation for this is that, due to the semantics of the \squo{until}, the verification of $\Phi_1$ has to be performed in every prefix of the run and, when $\Phi_1$ is a QoS constraint, each verification is done by calling Z3 with a different SMT-LIB query.
% 
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/evaluation/satisfiable-until}
        \caption{Satisfiable instances}
        \label{fig:eval:sat}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/evaluation/unsatisfiable-until}
        \caption{Unsatisfiable instances}
        \label{fig:eval:unsat}
    \end{subfigure}
    \label{fig:eval}
    \caption{Execution time to analyse (un)satisfiable \squo{until} formulas}
\end{figure}


\subsection{Nested choices}
\marginpar{Explain that we will measure the impact of nested choices over synthetic systems.}
%
We consider a system of two participants taking turns in sending a
message to each other; the sender of each turn chooses between two
messages.
%
Due to the branching nature of this behaviour, the number of runs of
the system grows as $2^n$ where $n$ is %%% an exponential of base 2 that depends on
the number of nested choices (i.e., the number of turns).
%
We synthetically generate systems with this behaviour by varying
$n$ %%% the number $n$ of nested choices
from 1 to 10.
%
Note that nested choices correspond to nested conditional statements
in a program and accepted software metrics
recommend %%% . However, this should not be a big issue in practice. In fact, standard practices and software metrics advise
to avoid large numbers of nested conditional statements.
%
In particular, an accepted upper bound of \emph{cyclomatic complexity}\footnote{
  %
  Cyclomatic complexity~\cite{mccabe:ieeetse-se-2_4} measures the complexity of programs according
  to the number of independent paths represented in the source code.
  %
} is 
15, which corresponds to less than 4 nested conditional statements.
%%% In particular, \emph{cyclomatic complexity} aims to measure the complexity of programs by reflecting the number of independent paths represented in the source code.
    % In~\cite{mccabe:ieeetse-se-2_4} the author draw conclusion of the application of this metric to programs in a production environment from which it can be read:
    % \begin{quote}
    % The particular upper bound that has been used for cyclomatic complexity is 10 which seems like a reasonable, but not magical, upper limit. 
    % \end{quote}
	 %%% A cyclomatic complexity~\cite{mccabe:ieeetse-se-2_4} of up to 10--15, a nowadays accepted upper bound, represents less than 4 conditiona statements, for independent conditions forming a sequence, or 14, for dependant conditions that can not be factored out.%, forming a perfectly balanced binary tree.

To generate these systems, we craft QoS-extended g-choreography in
\texttt{.qosgc} format and then leverage \chorgram's \texttt{G-chor
  projection} to obtain the qCFSMs of the system.
  %
The QoS specifications comprise five QoS attributes and determine 
unique values for them in each final state, enabling the
construction of $\QL$ formulas that are satisfied by only one run of
the system.  In this way, we can use these generated cases to evaluate
the performance of \thetool in finding the only run that satisfies a
formula in a search space of exponential size in $n$.
\begin{figure}[h]
  \begin{subfigure}{0.46\textwidth}
    \begin{lstlisting}[language=sgc,basicstyle=\scriptsize]
$\p[Bob]$ -> $\p[Alice]$: $\msg[m0]$ ; {
  $\p[Alice]$ -> $\p[Bob]$: $\msg[m0]$; $\p[Bob]$ -> $\p[Alice]$: $\msg[leaf1]$
  +
  $\p[Alice]$ -> $\p[Bob]$: $\msg[m1]$; $\p[Bob]$ -> $\p[Alice]$: $\msg[leaf2]$
}

+

$\p[Bob]$ -> $\p[Alice]$: $\msg[m1]$; {
  $\p[Alice]$ -> $\p[Bob]$: $\msg[m0]$; $\p[Bob]$ -> $\p[Alice]$: $\msg[leaf3]$
  +
  $\p[Alice]$ -> $\p[Bob]$: $\msg[m1]$; $\p[Bob]$ -> $\p[Alice]$: $\msg[leaf4]$
}
    \end{lstlisting}%
    \caption{Generated g-choreography for $n = 2$}
    \label{fig:eval:nested-choices-code}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.46\textwidth}
        \centering
        \includegraphics[scale=.33]{images/evaluation/nested-choices}
        \caption{Average execution time versus $n$}
        \label{fig:eval:nested-choices-plot}
    \end{subfigure}%
\caption{Performance on the `average' case for formulas with nested choices}
\label{fig:eval:nested-choices}
\end{figure}
The formula is generated by following the pattern
$\top\ \qluntil\ \psi$, were $\aG$ matches every run of the
system and $\psi$ is a QoS constraint, determining the value of the five QoS
attributes, that is satisfied by only one run.
%
In \cref{fig:eval:nested-choices-code} we show the generated $\aG$ for
two nested choices.
%
See \cref{appendix:nested-choices} for a detailed view of the 
files used in this case study.
% 
The bound \texttt{k} is set high enough to guarantee that all runs of
the system are reached by the analysis.  For each value of $n$, we
generate 100 different random instances of the $\QL$ formula, where
the only run that satisfies the formula is chosen randomly, and
execute \thetool on each instance. In
\cref{fig:eval:nested-choices-plot} we show the results as a boxplot
per number of nested choices.
%
Remarkably, both the average execution time and its variance grow as
$n$ increases.
%
This is due to the fact that the difference in time
between the best and worst case scenarios, where the model is found
either in the first or the last enumerated run matching $\aG$,
increases with $n$.
%
The apparent bias in dispersion towards lower
execution times is just a visual effect due to the logarithmic scale
of the y-axis.


\subsection{Model extraction}
\marginpar{Rewrite everything and explain example}
%
In this section we aim at evaluating the applicability of \thetool on a system of CFSMs
(see~\cref{fig:eval:kmclib}) inferred from the OCaml code of the case
study presented in~\cite{imai:tacas22}.

In the system of~\cref{fig:eval:kmclib} the user requests the master
to resolve a computational problem (whose nature is inconsequential
here).

In this case, we aim at evaluating how the complexity of the g-choreographies
indexing the \squo{until} affects the performance of \thetool.

The master splits the problem into two tasks and sends them to the
worker, which sends back to the master the solutions of each task.
%
Before collecting the second partial results from the
  worker, the master sends a \squo{work-in-progess} message to the
  user.
%
Finally, upon reception of the second partial result,
the master combines the solutions and sends the final result to the
user.
%
The thick gray arrow in~\cref{fig:eval:kmclib} is the only addition we
made to the original case study so to enable the user to decide to
iteratively make new requests or to stop.
%
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[node distance=0.5cm, every node/.style={scale=.8,transform shape,font=\scriptsize}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
        % User
        \node[cnode,initial, initial where = right, initial text=User] (u1) {};
        \node (u2) [cnode, below = of u1] {};
        \node (u3) [cnode, below = .7cm of u2] {};
        \node (u4) [cnode, right = of u3, double] {};
        \path[line] (u1) -- node[left]{$\aout[U][M][compute]$} (u2);
        \path[line] (u2) edge[bend left=-35] node[left]{$\ain[M][U][result]$} (u3);
        \path[line] (u3) edge[bend left=-35, color=gray, thick] node[right]{$\aout[U][M][compute]$} (u2);
        \path[line] (u3) -- node[below]{$\aout[U][M][stop]$} (u4);
        \path[line] (u2) edge [loop right] node[right]{$\ain[M][U][wip]$} (u2);
		\end{tikzpicture}
		\qquad
		% Master
		\begin{tikzpicture}[node distance=0.5cm, every node/.style={scale=.8,transform shape,font=\scriptsize}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
		  \node (m7) [cnode] {};
        \node (m6) [cnode, below = of m7] {};
        \node (m5) [cnode, below = of m6] {};
        \node (m4) [cnode, right = 1cm of m5] {};
        \node (m3) [cnode, right = 1.5 of m4] {};
        \node (m2) [cnode, above = of m3] {};
        \node (m1) [cnode, initial, initial where = right, initial text = Master, right = 3.5cm of m7] {};
        \node (m8) [cnode, right = 2cm of m4] {};
        \node (m9) [cnode, accepting, right = 1.5cm of m8] {};
        \path[line] (m1) -- node[left]{$\ain[U][M][compute]$} (m2);
        \path[line] (m2) -- node[above left = -.1cm]{$\aout[M][W][task]$} (m3);
        \path[line] (m3) -- node[below]{$\aout[M][W][task]$}  (m4);
        \path[line] (m4) -- node[below]{$\ain[W][M][result]$} (m5);
        \path[line] (m5) -- node[right]{$\aout[M][U][wip]$} (m6);
        \path[line] (m6) -- node[right]{$\ain[W][M][result]$} (m7);
        \path[line] (m7) -- node[above]{$\aout[M][U][result]$} (m1);
        \path[line] (m1) -- node[sloped, below]{$\ain[U][M][stop]$} (m8);
        \path[line] (m8) -- node[below]{$\aout[M][W][stop]$} (m9);
		\end{tikzpicture}
		\qquad
		% Worker
		\begin{tikzpicture}[node distance=0.5cm, every node/.style={scale=.8,transform shape,font=\scriptsize}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
        \node[cnode, initial, initial where = above, initial text=Worker] (w1) {};
        \node[cnode, below left = 1cm of w1] (w2) {};
        \node[cnode, below right = 1cm of w1, accepting] (w3) {};
        \path[line] (w1) edge[bend left=-35] node[above, sloped]{$\ain[M][W][task]$} (w2);
        \path[line] (w2) edge[bend left=-35] node[below, sloped]{$\aout[W][M][result]$} (w1);
        \path[line] (w1) -- node[sloped, above]{$\ain[M][W][stop]$} (w3);
        % \foreach \s/\l/\t in {0/\specA/1,1/{}/2}{
        %     \node (A\t) [cnode, right = of A\s, label = $\l$] {};
        % }
        % \node (A3) [cnode, right = of A2, fill = black] {};
        % \foreach \s/\l/\t in {0/\aout[a][b][x]/1,2/\aout[a][b][z2]/3}{
        %     \path[line,sloped] (A\s) edge node[below]{$\l$} (A\t);
        % }
        % \path[line] (A1) edge[bend left=-35] node[below]{$\ain[b][a][y]$} (A2);
        % \path[line] (A2) edge[bend left=-35] node[above]{$\aout[a][b][z1]$} (A1);
        \end{tikzpicture}
    \caption{Communicating system of the case study presented in \cite{imai:tacas22}}
    \label{fig:eval:kmclib}
\end{figure}
% \vspace{-0.5cm}

The QoS specifications involve \emph{p} (price), \emph{t} (number of
tasks computed) and \emph{pmem} (allocated memory); they have been manually specified and assigned to states
in the machines were they matter.
%
For instance, we model the problem instance to consume at most 5 units
of memory, thus consistently specify bounds on \emph{pmem} in the
states where a machine needs to allocate memory for the
problem. Similarly, we limit to one unit the memory needed for the
result, to ten units the price charged by the master once the
computation is done, while worker charges a cost that depends on the size of the
task.
%
Finally, we check the following $\QL$ properties of the model:
$$\begin{array}{lcl@{\qquad}lcl}
  \Phi_1 & \equiv & [\aG] (t \cdot 6 \leq p < 12.5)
   & \Phi_3  & \equiv & [\grec[][\aG]] (1 \leq \mathit{pmem} < 10)
  \\
  \Phi_2 & \equiv & [\grec[][\aG]] (t \cdot 6 \leq p < 12.5)
  & \Phi_4 & \equiv & (p \leq t \cdot 12.5)\ \qluntil ([\grec[][\aG]]\ p \leq 25) 
\end{array}$$
where $\aG$ describes the process of computing one problem instance, starting in
$\gint[][U][compute][M]$ and ending in $\gint[][M][result][U]$. 
% 
(See \cref{appendix:model-extraction} for a detailed view of the
files used in this case study.)
% 
Formula $\Phi_1$ uses the necessity modality to express bounds on the price
of the computation of one problem instance. Formulas $\Phi_2$ and $\Phi_3$
use the necessity modality to express bounds on the price and the memory used
after computing any number of problem instances. 
% 
We run \thetool on these three formulas and obtain a model within a bound \texttt{k} = 18, 
which is the length of the the runs that first match $\aG$ and then advance to a final configuration. 
In each case, \thetool is able to find the model in less than 0.4 seconds.
% 
By using the \texttt{validity} command we can also use \thetool as a counterexample finding procedure by checking satisfiability of the negation
of the formula. With a bound \texttt{k} = 32 it takes, respectively, 35, 206 and 208 seconds
to report that no counterexamples were found for $\Phi_1, \Phi_2$ and $\Phi_3$.
% 
Formula $\Phi_4$ states that
\begin{inparaenum}[1)]
    \item up to the computation of the first problem instance, the price falls below a bound depending on the number of tasks computed, and
    \item afterwards, the price is always bounded by 25 right after any number of computed problem
    instances.
\end{inparaenum}
Using a bound \texttt{k} = 18, it takes \thetool 0.7 seconds to find a model for $\Phi_4$.
If we use \thetool as a counterexample finding procedure, the bound is not enough
to find a counterexample: it takes 7 seconds to report that no counterexamples
were found. However, if we increase the bound to \texttt{k} = 32, \thetool finds a counterexample
in 35 seconds. Which shows that, unlike the previous formulas, $\Phi_4$ is satisfiable but it is not valid.

\hsl

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> introduction.tex <==
%!TEX root = ./main.tex

The way in which software systems are constructed and deployed has radically changed over the last decades. Nowadays software artifact are no longer monolithic constructions running in isolation. Instead, they can be though of as cooperating components, communicating on an adequate environment to perform its execution. Even more, there is a rapidly increasing number of software systems that are conceived, from its design stage, as a set of participants executing over globally available computational resources, and interacting with each other over existing communication infrastructure, in a distributed way in order to fulfill a collective goal.

There is big body of work versing on the problem of formalising the
communicating behaviour of distributed systems. Among those languages
choreographies stand out. Choreographic models of advocate a
\emph{global view} and a \emph{local view}.
%
The former is a high-level description of the interactions among
components that abstracts away some aspects in order to offer a
holistic understanding of the communication behaviour of the
system.
%
The latter view is a description of each component in isolation.
%
% They can be described both from a global point of view (see \eg~\cite{denielou:esop12} or from a local point view (i.e., the standpoint of each individual component) (see \eg~\cite{brand:jacm-30_2}, and for which there exists associated analysis methods like synthesis of \emph{Global graphs} from \emph{Communicating Finite State Machines} (CFSMs) \cite{lange:popl15} that can be applied in order to determine realisability free from communication errors or conformance of a component's behaviour to a protocol \cite{vissani:places15}.

With the flourishing of ubiquitous computing and the emergence of more
dynamic computing paradigms such as Cloud/Fog/Edge Computing, Service
Oriented Computing and, what is sometimes referred to as, the API's
economy~\cite{dwasl16,apiIBM}, reasoning about the QoS of the
components has become a key issue in the design and execution of
distributed systems.
%
In previous work~\cite{martinezsune:coordination19} we have proposed an automatically analysable specification language for QoS where contracts are captured as constraints over quantitative attributes of interest (\eg~computation time required, storage required, waiting time, cost, etc.). Such specifications can be thought of as logical characterisations of the admisible values of the quantitative attributes of the software component along its executions.

When software components are observed from the standpoint of their communication behaviour (\eg~when they are specified through the use of languages like CFSMs) we access a different, one could say more internal, view of how the computation is performed. From this viewpoint a component's computation can be rationalised along a run whose states correspond to states of the CFSM, and describe bits of the computation, linked by the communication actions. Therefore, we can naturally extend the language of the CFSMs by attaching QoS constracts to the states, describing the cost associated to the computation performed in them.

\eMcomm{
  should we claim that this is the first framework of behavioural types with QoS
}{Our main contributions are as follows.}

\begin{itemize}
\item A modelling language to express QoS attributes of components.
  %
  The language is straightforwardly attained by the states of CFSMs
  with constraints specifying QoS aspects of local computations.
  %
  This design decision assumes that there is no control on communication
  infrastructure.
  %
  More precisely, QoS aspects related to how communications are
  realised are not under the control of applications' designers.
  %
  Instead, designers have control on local computation, thus
  suggesting that QoS constraints are naturally associated to states
  of CFSMs.
  %
  We decided to adopt real-closed fields to represent QoS values;
  besides being a complete and decidable abstract formalisation of the
  real numbers, real-closed fields are instrumental for a smooth
  definition of our framework.
  % %
  % In particular, real-closed fields (and their extensions
  % to express QoS constraints) can be conveniently defined as
  % presentations of first-order theories.
\item A logical language for describing QoS properties of interest of
  communicating systems.
  %
  Our logic, dubbed $\QL$, is inspired by \emph{Propositional Dynamic
	 Linear Temporal Logic} (DLTL) \cite{henriksen:apal-96_1_3}.
  %
  A distinct characteristic of $\QL$ is that it indexes temporal
  modalities with \emph{g-choreographies}~\cite{tuosto:jlamp-95}, a
  model of global views of choregraphies, in order to predicate on QoS
  properties of the whole system.
  %
  Noteworthy, we could not directly use $\DLTL$ for our
  purposes.
  %
  This is due to two limitations shortcomings.
  \begin{inparaenum}[1)]
  \item The satisfiability of a $\DLTL$ formula relies on the
	 prefixes of runs being checked to belong to the language of the
	 regular expressions.
	 %
	 In our case, this is not enough; as it will become clear in
	 \cref{sec:logic} (cf. \cref{def:aggregation-function} and
	 \cref{def:ql-semantics}), in our proposal, satisfaction will
	 require collecting information along the prefix of \emph{maximal}
	 runs.
  \item In $\DLTL$ modalities are indexed by regular
	 expressions over atomic actions.
	 %
	 In our case, this would mean to use an alphabet of output and
	 input actions.
	 %
	 However, global views of choregraphies (such as g-choreographies)
	 hinge on \emph{interactions}, an abstraction to represent
	 handshakes between a sender an a receiver.
	 %
	 Also, such interactions are then realised asynchronously thus
	 breaking the atomicity.
  \end{inparaenum}
\item \eMcomm{}{I'll expand this} A decision procedure for checking
  satisfiability of QoS properties by a communicating system.
\end{itemize}
These contributions collectively constitute a framework achieving what
we believe is a crucial need of modern distributed computational
models like those mentioned before.

The paper is organised as follows: in Sec.~\ref{sec:pre} we provide
the formal definitions regarding communicating systems and the
specification of quantitative attributes that will use in the rest of
the paper; in Sec.~\ref{sec:QoS-choreo} we present the main
contribution of the paper, a QoS extension of communicating machines
and a logical language to express QoS properties, together with an
analysis algorithm presented in \cref{sec:analysis}. Finally, in
Sec.~\ref{sec:conclu} we draw some conclusions and point out some
further lines of research.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> logic.tex <==
% !TEX root = ./main.tex
%
% In the quest for defining a methodology for QoS-aware message-passing
% distributed systems design and analysis, once we provided a language
% for describing the system, a formal language for stating the desired
% properties is needed. For instance, one could be interested in analysing 
% the monetary cost of the client component in the communicating system
% for the POP protocol (cf.~\cref{ex:pop}).
%
To describe QoS properties we introduce $\QL$, a logical language akin
$\DLTL$.
%
% The syntax of $\QL$ differs from the syntax of $\DLTL$ just on the indexes of temporal modalities.
%
\begin{definition}[QoS formulae]\label{def:globalQoSprop}
  The \emph{QoS logic} $\QL$ consists of the smallest set of
  formulae that can be obtained from the following grammar:
  \begin{align*}
    % \aG & \bnfdef & \gempty \bnfmid \gint[] \bnfmid \gseq[] \bnfmid \gpar[] \bnfmid \gcho[] \bnfmid \grec[][@][]\\
    \gqosprop & \bnfdef \top \bnfmid \psi \bnfmid \neg \gqosprop \bnfmid \gqosprop \lor \gqosprop \bnfmid \gqosprop\ \qluntil \gqosprop
  \end{align*}
  where $\psi$ is a formula in a theory presentation in
  $\qosspecs$, and $\aG$ is a g-choreography over 
  $\PSet$ and $\msgset$ (see \cref{def:g-choreography}).
  % If $\aG$ is free from any $\grecop$ operators (see \cref{def:g-choreography})
  % We write $\QL^\grecop$ for the extension of $\QL$ where $\grecop$ is allowed.
\end{definition}
%
Atomic formulae express constraints over quantitative attributes.
%
Akin $\DLTL$, properties of runs are linear temporal formulae
where the until operator is indexed with a global choreography
 $\aG$. In essence, the role of $\aG$ is to restrict the set of
  runs to be considered for the satisfiability of the until.
  Global choreographies are suitable for this purpose because they
  are a declarative and compact way of characterizing the behaviour 
  of asynchronous message-passing systems.
%
The possibility modality $\conf \aG \gqosprop$ is defined as
$\top \qluntil \gqosprop$ and the necessity modality
$[\aG] \gqosprop$ is defined (dually) as
$\neg \conf \aG \neg \gqosprop$.
%
Finally, propositional
connectives $\land$ and $\implies$ are defined as usual.

The following example shows how to express non-functional properties
of specific runs of the system in $\QL$.
%
\begin{example}[QoS properties of POP protocol]\label{ex:qos-prop}
  % We can use $\QL$ to specify relations between the monetary cost
  % and the resources consumed.
  %
  We can use the g-choreographies and the $\QL$ formula below to state
  that, unless the cost is zero for the first three e-mails read, the
  cost is bounded by $10$ times the CPU time, and the memory
  consumption is bounded by $5$.
  %
  We define
  \begin{align*}
	 \gqosprop \equiv &\ [\aG_3]( c > 0 ) \implies [\aG_3;{\grec[][\aG_{\mathsf{msg}}]}]\big( ( c \leq t \cdot 10 ) \land (m \leq 5) \big)
							  \qqand[where]
	 \\	 
    \aG_3 = &\ \gint[][c][helo][s]; \gint[][s][int][c];\aG_{\mathsf{msg}};\aG_{\mathsf{msg}};\aG_{\mathsf{msg}} \qqand
	 \\
    % \aG_{4+} = &\ \aG_3;{\grec[][\aG_{\mathsf{msg}}]} \\
    \aG_{\mathsf{msg}} = &\ \gint[][c][read][s]; \gint[][s][size][c]; \gint[][c][retr][s]; \gint[][s][msg][c]; \gint[][s][ack][c]
  \end{align*}
  % 
  Intuitively, for $\gqosprop$ to hold, either the first three message
  retrievals must have zero cost in any run of the system, or on every
  subsequent message retrieval, the total cost and memory consumption
  fall within the specified bounds.
  %
  \finex
\end{example}

A $\QL$ formula (like $\gqosprop$ in \cref{ex:qos-prop}) can be used
in quantitative analyses by \emph{aggregating} the values of the QoS
attributes along the runs of the system.
%
More precisely, given a run
$\pi$, our interpretation is that, for each transition $s_i \TRANSS{\al_i} s_{i+1}$ of $\pi$, the
obligations stated in the QoS specification of $s_i$ are met after
aggregating QoS information along $\pi$ from state $s_0$ up to state
$s_i$.
Therefore, a central notion in our framework is that of \emph{aggregation function}.
% \begin{definition}[Aggregation function]\label{def:aggregation-function}
%   Let $\aCS$
%   %  = (\conf{ \aCM_p, \qos_{\p}})_{\p \in \PSet}$ 
%    be a QoS-extended communicating system.
%   %
%   Given
%   $\pi
%   %  = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots
%   % \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n} 
%   \in
%   \Delta_{\aCS}$, an \emph{aggregation function}
%   has the signature $\aggfn_{\aCS} : \Delta_{\aCS} \to \qosspecs$. 
%   For every run in the system, it produces a QoS specification 
%   that captures the aggregated QoS attributes by considering the QoS 
%   specifications of the participants' local states.
% \end{definition}
Given a QoS-extended communicating system
$\aCS$, an \emph{aggregation function} $\aggfn_{\aCS} : \Delta_{\aCS}
\to
\qosspecs$ yields a QoS specification capturing the cumulative QoS
attributes along a run $\pi
  %  = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots
  % \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n} 
  \in
  \Delta_{\aCS}$ by \quo{summing-up} QoS specifications of participants' local states.
%
% In the following, we illustrate the specific aggregation function we use in our framework by means of an example.
\begin{example}[Aggregation]\label{ex:aggregation}
  Recall the run $\pi$
  \eqref{eq:idea} from \cref{sec:intro}:
  %
  \begin{align*}
	 \begin{tikzpicture}[node distance = .5cm and 3cm, every node/.style={font=\scriptsize}, every label/.style={color=blue,fill=yellow!10}]
		\node[label={above:$\{ c \leq 5, m = 0 \}$}] (aq0) {$\aQzero$};
		\node[left = 1cm of aq0] {\p:};
		\node[right = of aq0, label={above:$\{ 5 \leq c \leq 10,\ m < 3 \}$}] (aq1){$q_1$};
		\path[->,draw] (aq0) edge node[above] {$\aout$} (aq1);
		\node[below = of aq0, label={above: $\{c=0,m=0\}$}] (bq0){$\aQzero'$};
		\node[left = 1cm of bq0] {\q:};
		\node[right = of bq0, label={above:$\{10 \leq m \leq 50,\ c = 0.01 \cdot m \}$}] (bq1){$q_1'$};
		\path[->,draw] (bq0) edge node[above] {$\ain$} (bq1);
		\node(s0) [below = of bq0]{$\aConf_0$};
		\node[left = 1cm of s0] {$\pi$:};
		\node[right = of s0] (s1){$\aConf_1$};
		\node[right = of s1] (s2){$\aConf_2$};
		%
		\path[->,draw] (s0) edge node[above] {$\aout$} (s1);
		\path[->,draw] (s1) edge node[above] {$\ain$} (s2);
	 \end{tikzpicture}
  \end{align*}

  % \begin{equation}\label{eq:idea}
  %   \begin{array}{l@{:\qquad}l}
  %   \text{behaviour of \p} &
  %   \begin{tikzpicture}[node distance = 1cm and 4cm, every node/.style={font=\scriptsize}, every label/.style={color=blue,fill=yellow!10}]
  %    \node[label={above:$\{ c \leq 5, \mathit{mem} = 0 \}$}] (aq0) {$\aQzero$};
  %     \node[right = of aq0, label={above:$\{ 5 \leq c \leq 10,\ \mathit{mem} < 3 \}$}] (aq1){$q_1$};
  %    \path[->,draw] (aq0) edge node[above] {$\aout$} (aq1);
  %   \end{tikzpicture}
  %   \\[2em]
  %   \text{behaviour of \q} &
  %   \begin{tikzpicture}[node distance = 1cm and 4cm, every node/.style={font=\scriptsize}, every label/.style={color=blue,fill=yellow!10}]
  %     \node[label={above: $\{c=0,\mathit{mem}=0\}$}] (bq0){$\aQzero'$};
  %     \node[right = of bq0, label={above:$\{10 \leq \mathit{mem} \leq 50,\ c = 0.01 \cdot \mathit{mem} \}$}] (bq1){$q_1'$};
  %    \path[->,draw] (bq0) edge node[above] {$\ain$} (bq1);
  %   \end{tikzpicture}
  %   \end{array}
  % \end{equation}


  %
  Let $c_{\p}^q$ (resp. $c_{\q}^q$) denote the value of the QoS
  attribute $c$ in the state $q$ of participant \p\ (resp. \q) and
  likewise for the attribute $\mathit{m}$.
  %
  After $\pi$, we expect
  % \begin{align*}
	 $\max{\{m^{q_0}_{\p}, m^{q_1}_{\p}, m^{q'_0}_{\q}, m^{q'_1}_{\q}\}}$
   and
	%  \qqand
	 $c^{q_0}_{\p} + c^{q_1}_{\p} + c^{q'_0}_{\q} + c^{q'_1}_{\q}$
  % \end{align*}
  to respectively be the memory consumption and the overall monetary 
  cost in $s_2$.
  %
  This boils down to aggregate the QoS attributes $c$ and
  $m$ using the maximization and addition operations, respectively.
  %
  \finex
\end{example}

% 
%
% \begin{figure}[ht]
%   \centering
%   \begin{tikzpicture}[node distance = 1cm and 4cm]
% 	 \node[label={$\begin{array}{l}
% 						  \{ t_\mathit{exe} \leq 5*t_\mathit{wait} + m^3,\\
%                   \ \ t_\mathit{wait} < 10 \}
%                 \end{array}$
%               }] (aq0) {$\aQzero$};
%     \node[right = of aq0, label={$\begin{array}{l}
%                                   \{ t_\mathit{wait} < 5, \\
%                                   \ \ t_\mathit{exe} \leq 20 \}
%                                 \end{array}$}] (bq0){$\aQzero$};
%     \node[below = of aq0, label={below:$\begin{array}{l}
%                   \{ t_\mathit{wait} = 0,\\
%                   \ \ t_\mathit{exe} \leq 10 \}
%                 \end{array}$
%               }] (aq1){$q_1$};
%     \node[below = of bq0, label={below:$\begin{array}{l}
%                   \{ t_\mathit{wait} < 2,\\
%                   \ \ m * \log(m) \leq t_\mathit{exe} \leq m^2 \}
%                 \end{array}$
%               }] (bq1){$q_1$};
%     \node[right = of bq0,label={above:$\pi$}] (path){$((\aQzero,\aQzero);(\epsilon,\epsilon))$};
%     \node[below = .7cm of path] (path1) {$((q_1,\aQzero);([\msg],\epsilon))$};
%     \node[below = .7cm of path1] (path2) {$((q_1,q_1);(\epsilon,\epsilon))$};
%     \node at (-1,-1) {$\aM_{\p}$};
%     \node at (6,-1) {$\aM_{\q}$};
%     %
% 	 \path[->,draw] (aq0) edge node[above,sloped] {$\aout$} (aq1);
% 	 \path[->,draw] (bq0) edge node[above,sloped] {$\ain$} (bq1);
% 	 \path[->,draw] (path) edge node[right] {$\aout$} (path1);
% 	 \path[->,draw] (path1) edge node[right] {$\ain$} (path2);
%   \end{tikzpicture}
%   \caption{Aggregation\label{fig:ex:accumulation}\label{fig:ex-cfsms}}
% \end{figure}
% Participant $\p$ performs a computation from state $\aQzero$ whose QoS
% contracts restricts the waiting time $t_\mathit{wait}$, the execution
% time $t_\mathit{exe}$, and the $m$ of data; in state $q_1$
% the QoS contract of $\p$ changes as shown in
% \cref{fig:ex:accumulation}. And likewise for $\q$. The semantics of
% this simple system is the run $\pi$ in the rightmost part of
% \cref{fig:ex:accumulation}.
% %
% Run $\pi$ simply connects three configurations with the action of
% sending the message $\msg$ from participant $\p$ to participant $\q$,
% and its corresponding reception.
% %
% Take the property
% $\gqosprop_t = \conf{\gint[]} \left(t_\mathit{wait} + t_\mathit{exe}
%   \leq m^3 + m^2 + 150 \right)$ stating a
% bound for the time spent in the execution of the interaction
% $\gint[]$.
% %
% % The reader should note that the LTS $\msgset_{\{\p, \q\}}$ of
% % \cref{fig:ex-cfsms} is, at the same time, the only run of the
% % communicating system $\{\p, \q\}$ of \cref{fig:ex-cfsms} and that,
% % intuitively, it is legal for the program
% % $\p \stackrel{\mathsf{m}}{\longrightarrow} \q$. 
% % Let $\pi$ be such run;
% % 
% To check the satisfaction of $\gqosprop_t$ the value of the attributes
% must be considered by \quo{aggregating} the constraints on them along
% the executed run.
% %
% For instance, $t_\mathit{wait}$ and $t_\mathit{exe}$ in our example
% must satisfy different conditions in each local state of $\p$ and
% $\q$.
% %
% As said earlier, the aggregation operation depends on the nature of
% the attributes; for simplicity, we use addition\footnote{This yields
% an over-approximation as it does not consider the potential
% overlapping of time across different machines on a truly concurrent
% system.
%   % , but this is consistent with the fact that such an overlapping
%   % might not take place, and there is no way to enforce it.
%   More sophisticated aggregation operations could provide more precise
%   abstractions.  } to aggregate the time attribute $t$ and maximum for
% the memory attribute $m$.
%
% Under this interpretation of QoS attributes, if $c^{q}_{\p[x]}$ is the
% attribute $c$ in state $q$ of participant $\p[x]$, at the end of a run
% we expect that $m$ remains constant (i.e.
% $m = {m}^{\aQzero}_{\p} =
% {m}^{q_1}_{\p} = {m}^{\aQzero}_{\q} =
% {m}^{q_1}_{\q}$) and that
% $t_\mathit{wait} = {t_\mathit{wait}}^{\aQzero}_{\p} +
% {t_\mathit{wait}}^{q_1}_{\p} + {t_\mathit{wait}}^{\aQzero}_{\q} +
% {t_\mathit{wait}}^{q}_{\q}$ (and likewise for $t_\mathit{exe}$).
%
% In order to formalise the aggregation operation over execution paths
% of a communicating system, we substitute QoS attributes in the QoS
% constraints associated to a specific configuration of a participant
% with (fresh) symbols so the values they adopt are uniquely related to
% that specific computation. This is done by decorating the QoS
% attributes of a formula as in the previous example.
%
% The value associated to a specific QoS attribute in a run of the
% system results from aggregating the different incarnations of
% corresponding QoS attribute from each configuration occurring along
% the run; this is done using the aggregation operator corresponding to
% that specific attribute.
%
Essentially, the aggregation in this case is obtained by
(1) instantiating the QoS specification associated to the local state
  of participants
  (this is done by renaming attributes as in \cref{ex:aggregation}); and
(2) adding an equation combining all the instances of QoS specifications.
%
The following formula captures this intuition
  and exemplifies one way in which the aggregation function could be defined.

% \begin{eMenv}[Meta-comment]
%   %
%   I think we need more precision on aggregation:
%   \begin{itemize}
%   % \item shouldn't $\psiinst[c][@][\vec{q}(\p)]$
% 	%  be $\psiinst[c][@][\vec{q}_0(\p)]$ in the first case of $g$?
%   % \item $f$ and $g$ do not yield members of $\qosspecs$ (the declared codomain of $\aggfn$ is the class of qos specifications, cf. \cref{def:qos-spec})
%   % \item I think  operations must be binary associative internal operations.
%   \item The comment on parallel vs sequential after \cref{def:aggregation-function} hints that we don't need parallel composition
%   \end{itemize}
%   % 
% \end{eMenv}
%
% 
% 
\begin{example}[Aggregation]\label{ex:aggregation-function}
  Let $\aCS = (\conf{ \aCM_{\p}, \qos_{\p}})_{\p \in \PSet}$,
  we define the aggregation function 
  $\aggfn_{\aCS} : \Delta_{\aCS} \to \qosspecs$ to be
  $\aggfn_{\aCS} (\pi) = f(\pi) \cup g(\pi)$ where
  \begin{align*}
	 f(\pi) = & \bigcup\limits_{\substack{\p \in \PSet\\0 \leq i \leq n}} \psiinst[\qos_{\p}({{\vec q_i}(\p)})][@][{{\vec q_i}(\p)}]
	 \qqand
	 g(\epsilon) = %&
		\left\{ \genericAttr = \left(\bigoplus^{\quad \genericAttr}\limits_{\substack{\p \in \PSet}} \psiinst[\genericAttr][@][{\vec q_0}(\p)]\right) \sst \genericAttr \in \constset[Q] \right\} % & \text{if } n =0
		\\
   g(\pi) = &
		\left\{ \genericAttr = \left(\bigoplus^{\quad \genericAttr}\limits_{\substack{0 \leq i < n\\ \p = {\subject[\al_i]}}} \psiinst[\genericAttr][@][{\vec q_i}(\p)]\right) \oplus^\genericAttr \left(\bigoplus^{\quad \genericAttr}\limits_{\substack{\p \in \PSet}} \psiinst[\genericAttr][@][{\vec q_n}(\p)]\right) \sst \genericAttr \in \constset[Q] \right\}
		% \qquad\qquad\qquad\qquad\qquad\quad \mbox{; if $\pi = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n}$}
		\qquad \text{if } \pi \not\eq \epsilon
	%  g(\pi) = & \begin{cases}
	% 	\left\{ c = \left(\bigoplus^{\quad c}\limits_{\substack{\p \in \PSet}} \psiinst[c][@][{\vec q_0}(\p)]\right) \sst c \in \constset[Q] \right\} & \text{if } n =0
	% 	\\
	% 	\left\{ c = \left(\bigoplus^{\quad c}\limits_{\substack{0 \leq i < n\\ \p = {\subject[\al_i]}}} \psiinst[c][@][\vec{q_i}(\p)]\right) \oplus^c \left(\bigoplus^{\quad c}\limits_{\substack{\p \in \PSet}} \psiinst[c][@][\vec{q_n}(\p)]\right) \sst c \in \constset[Q] \right\}
	% 	% \qquad\qquad\qquad\qquad\qquad\quad \mbox{; if $\pi = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n}$}
	% 	& \text{otherwise}
	% 	\end{cases}
  \end{align*}
where 
$\pi = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots
  \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n} \in
  \Delta_{\aCS}$,
  and
$\psiinst[\Pi] = \{\psiinst \sst \psi \in \Pi\}$ for a set of $\QL$ formulae $\Pi$, and $\psiinst$ is obtained by replacing each QoS attribute $c$
with the symbol $c_{\p}^q$ in the atomic formula $\psi$.
  The intuition is that $f(\pi)$ collects all the QoS specifications of the
  local states of the participants along the run $\pi$, and $g(\pi)$
  uses the aggregation operators to calculate the aggregated values of
  the QoS attributes in the run $\pi$. If we apply this aggregation
  function to the run $\pi$ in \cref{ex:aggregation}, we obtain the
  following:
  \begin{align*}
    f (\pi) =\ & \{ c^{\aQzero}_{\p} \leq 5, m^{\aQzero}_{\p} = 0 \} \cup \{ 5 \leq c^{q_1}_{\p} \leq 10,\ m^{q_1}_{\p} < 3 \}\\
    & \cup \{c^{\aQzero'}_{\q}=0,m^{\aQzero'}_{\q}=0\} \cup \{10 \leq m^{q_1'}_{\q} \leq 50,\ c^{q_1'}_{\q} = 0.01 \cdot m^{q_1'}_{\q} \} \\
    g (\pi) =\ & 	\left\{m = \max{\{m^{q_0}_{\p}, m^{q_1}_{\p}, m^{q'_0}_{\q}, m^{q'_1}_{\q}\}}, c = c^{q_0}_{\p} + c^{q_1}_{\p} + c^{q'_0}_{\q} + c^{q'_1}_{\q}\right\}
    \qquad\qquad\hfill\diamond
  \end{align*}
% The following auxiliary notation is useful:
% for an atomic $\QL$ formula $\psi$ and a state $q$ of the CFSM of a
% participant $\p \in \PSet$ of a QoS-extended communicating system, let
% $\psiinst$ be obtained by replacing each QoS attribute $c$
% with the symbol $c_{\p}^q$ which we also assume to be a QoS attribute.
% 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Old version.
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
%  \begin{align*}
% \aggfn (\pi) =
%	   	 \begin{cases}
%		\left(\bigcup\limits_{\substack{\p \in \PSet}} \psiinst[\qos_{\p}({\vec{q_i}(\p)})][@][{\vec{q}(\p)}] \right) \cup \left\{ c = \left(\bigoplus^{\quad c}\limits_{\substack{\p \in \PSet}} \psiinst[c][@][\vec{q}(\p)]\right) \sst c \in \constset[Q] \right\} \\
%		\qquad\qquad\qquad\qquad\qquad \mbox{; if $\pi = \conf{\vec q \, ; \, \vec b}$}\\
%		\left(\bigcup\limits_{\substack{0 \leq i < n\\ \p = {\subject[\al_i]}}} \psiinst[\qos_{\p}({\vec{q_i}(\p)})][@][{\vec{q_i}(\p)}] \right) \cup \\
%		\qquad\qquad\qquad\qquad \left\{ c = \left(\bigoplus^{\quad c}\limits_{\substack{0 \leq i < n\\ \p = {\subject[\al_i]}}} \psiinst[c][@][\vec{q_i}(\p)]\right) \oplus^c \left(\bigoplus^{\quad c}\limits_{\substack{\p \in \PSet}} \psiinst[c][@][\vec{q_n}(\p)]\right) \sst c \in \constset[Q] \right\} \\
%		\qquad\qquad\qquad\qquad\qquad \mbox{; if $\pi = \conf{\vec q_0 \, ; \, \vec b_0} \TRANSS{\al_0} \dots \TRANSS{\al_{n-1}} \conf{\vec q_n \, ; \, \vec b_n}$}
%		\end{cases}
%  \end{align*}
%  %
%  where, $\psiinst[\Pi] = \{\psiinst \sst \psi \in \Pi\}$ for a set of
%  $\QL$ formulae $\Pi$,
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{example}
%
% \eMcomm[Not clear]{The fact that $\aggfn$ takes a run of the system as input evidences that the notion
% of aggregation it captures is sequential rather than parallel.} 
It is important to emphasize that, in our conception, an aggregation
function relies on a run of the system as its input.  This run
inherently encompasses a specific sequential ordering of the actions
carried out by the participants.  The aggregation operators $max$ and
$+$ used in \cref{ex:aggregation} follow this interpration. As will
become clear in \cref{def:ql-semantics}, this interpretation is
sufficient for the purposes of this paper, since it enables $\QL$ to
specify temporal QoS properties about runs of the system.  However,
one might be interested in a different kind of aggregation that is
aware of local states that are executed in parallel. This may require
some care and possibly to exploit truly-concurrent models, such as
pomsets; this is left for future work.
% 
 
% Aggregation functions are a key ingredient in our framework.
The semantics of our logic is defined in terms of QoS-extended
communicating systems.
%  , and
% Which is defined in terms of Kripke structures \cite{kripke:zmlgm-9_56}
% \anote{This doesn't seem true, we define it in terms of a QoS-extended communicating system.}
%  assuming an entailment relation
% $\vdash_{\mathit{RCF}}$ % of a complete calculus for RCFs
% to handle atomic formulae.
%
% We only consider maximal runs \eMcomm[this is not true]{since those
% represent the observable behaviour of the system.}
%
% A run
%   $\pi \in \Delta^\infty_{\aCS} $ is \emph{maximal} if for all
%   $\pi' \in \Delta^\infty_{\aCS}$, if
%   $\pi \in \mathit{prf}(\pi')$ then $\pi' = \pi$.

\begin{definition}[$\QL$ semantics]\label{def:ql-semantics}
  % A run is \emph{terminating} if its last configuration is a final
  % conf. (see \cref{def:cfsm-extend}).
  %
  Given a QoS-extended communicating system $\aCS$, an
  \emph{$\aCS$-model for a QoS property $\gqosprop$} is a pair
  $\conf{\pi, \pi' }$, where $\pi \in \Delta^\infty_{\aCS}$ contains
  a final configuration 
  % $\csconf q \abuffer$
  (see \cref{def:cfsm-extend})
   and $\pi' \in \mathit{prf}(\pi)$ up to such configuration such that
  $\conf{\pi,\pi'} \models_{\aCS} \gqosprop$ where the %satisfaction
  relation $\models_{\aCS}$ is defined as follows:
  $$
  \begin{array}{rcl}
    \conf{\pi, \pi'} \models_{\aCS} \gqosprop & \mbox{ iff } & \aggfn_{\aCS} (\pi') \vdash_{\mathit{RCF}} \gqosprop \ \ \text{ if } \gqosprop \text{ is an atomic formula}\\ 
    \conf{\pi, \pi'} \models_{\aCS} \neg \gqosprop & \mbox{ iff } & \conf{\pi, \pi'} \models_{\aCS} \gqosprop \text{ does not hold}\\ 
    \conf{\pi, \pi'} \models_{\aCS} \gqosprop_1 \lor \gqosprop_2 & \mbox{ iff } & \conf{\pi, \pi'} \models_{\aCS} \gqosprop_1 \mbox{ or } \conf{\pi, \pi'} \models_{\aCS} \gqosprop_2\\ 
    \conf{\pi, \pi'} \models_{\aCS} \gqosprop_1\ \qluntil\ \gqosprop_2 & \mbox{ iff } & \text{there exists } \pi'' \text{such that } \rlang[\pi''] \in \hat{\rlang}[\aG], \\
    & & \pi'\pi'' \in \mathit{prf}(\pi) \text{ up to a final configuration in $\pi$,} \\
     & & \conf{\pi, \pi'\pi''} \models_{\aCS} \gqosprop_2 \text{ and, for all } \pi''' \in \mathit{prf} (\pi''),\\
     & & \text{if } \pi''' \neq \pi'' \text{ then } \conf{\pi, \pi'\pi'''} \models_{\aCS} \gqosprop_1.
  \end{array}
  $$

  \noindent
  A QoS property $\gqosprop$ is \emph{satisfiable} in $\aCS$ if there
  exists a run $\pi \in \Delta^\infty_{\aCS}$ such that
  $\conf{\pi, \epsilon} \models_{\aCS} \gqosprop$, and it is
  \emph{valid} (denoted as $\models_\aCS \gqosprop$) if, for all runs
  $\pi \in \Delta^\infty_{\aCS}$ that contain a final configuration,
  $\conf{\pi, \epsilon} \models_{\aCS} \gqosprop$.
\end{definition}
%
Negation and disjunction are handled in the standard way.
% 
The definition of the until operator is similar to the standard
operator: $\gqosprop_2$ must hold at some point in the future,
i.e., $\pi'\pi''$ and $\gqosprop_1$ must hold up to that point; the
key difference is that the satisfaction of $\gqosprop_2$ is restricted
to runs where the extension $\pi''$ is in $\hat{\rlang}[\aG]$.
% the language of $\aG$.
%
Finally, atomic formulae are handled by obtaining the aggregated QoS
of the accumulated run $\pi'$ and using the entailment relation of
RCFs.
% 
% \eMcomm[later?]{It is worth noting that, as usual, checking validity of a formula
% $\gqosprop$ (in a language that has negation) can be reduced to
% checking the satisfiability of $\neg\gqosprop$.
% }
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> methodology.tex <==
% !TEX root = ./main.tex

% We now present our methodology for the design of QoS-aware distributed
% systems.
%
Our methodology provides the means to statically analyse the satisfaction of QoS
properties of the overall system by relying on the QoS constraints specified for
its components.
%
The methodology consists of the following steps:
\begin{enumerate}
\item\label{it:gc} Identify a g-choreography modelling the global view of the
  system.
\item\label{it:cfsm} Determine a CFSM for each participant.
\item\label{it:qos} Identify relevant QoS attributes and the corresponding QoS
  constraints from the SLAs of each component.
\item\label{it:qcfsm} Assign QoS specifications to states within the CFSMs from the QoS constraints identified on step~\ref{it:qos}.
\item\label{it:ql} Specify the QoS property of interest of the system in the logic $\QL$.
\item\label{it:mc} Verify the QoS property.
\end{enumerate}
%
To describe the steps of our methodology we appeal to a simple yet
realistic scenario elaborating on the pop protocol presented in
\cref{sec:pre}; more precisely we consider a multi-party variant of
the protocol where a third-party service \p[a], modelled
after the \emph{OAuth} authentication protocol~\cite{rfc6749}, is used to authenticate
mail clients \p[c] to the POP server \p[s].

\noindent\textbf{Step \ref{it:gc}} We define the g-choreography
$\aG_{\mathsf{auth}}$ of the system as follows:
\begin{lstlisting}[language=sgc, basicstyle=\footnotesize]
  $\aG_{\mathsf{auth}}$ = $\ \gint[][c][cred][a]$;($\gcho[][{\aG_{\mathsf{token}}}][{\gint[][a][error][c]}]$)
  $\aG_{\mathsf{token}}$ = $\ \gint[][a][token][c]$;$\gint[][c][token][s]$;($\gint[][s][fail][c]$ + $\ \gint[][s][ok][c]$;$\aG_{\mathsf{POP}}$)
\end{lstlisting}
where $\aG_{\mathsf{POP}}$ is as in \cref{ex:gc-pop}.
%
The authentication server \p\ certifies the identity of the client
\ptp[c]; on successful authentication, \p\ hands out an authentication
token to \ptp[c] otherwise an error is notified and the protocol
terminates.
%
In the former case, \ptp[c] sends the authentication token to the
server to prove its identity; if the token is valid \ptp[s] sends
message $\msg[ok]$ to the client and the protocol continues as
specified by $\aG_{\mathsf{POP}}$; otherwise, \ptp[s] sends message
$\msg[fail]$ and the protocol terminates.

We note that the g-choreography does not necessarily need be written
manually; it can also be inferred out of local specifications using
algorithms such as those in~\cite{LT10,lange:popl15,clm17}.


\noindent\textbf{Step \ref{it:cfsm}} This step is instrumental
to Step \ref{it:qcfsm} since our methodology requires to specify the
qCFSM of each component of the system.
% , that will be passed to \thetool as a \texttt{.qosfsa} file.
As anticipated in \cref{sec:pre}, this requires first to have the set
of CFSMs that model the behaviour of the system and then to assign QoS
specifications to the states of each CFSM.
%
The CFSMs that are not already available can be inferred from code
(cf.  \cref{sec:eval}) or attained through \chorgram's \texttt{G-chor
  projection} feature that automatically derives the CFSMs for the
system's participants.
%
For example, the \aGcomm[check projection]{CFSMs shown below} are
obtained by projecting the g-choreography $\aG_{\mathsf{auth}}$ onto
the participants $\ptp[A]$, $\ptp[C]$, and $\ptp[S]$:
\begin{align*}
    \begin{tikzpicture}[node distance=.3cm and 1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (0) {};
        \node[cnode,right = of 0] (1) {};
        \node[cnode,above right = of 1] (2) {};
        \node[cnode,below right = of 1] (3) {};
%
        \path[line] (d) -- (0);
        \path[line] (0) edge node[below]{$\ain[c][a][cred]$} (1);
        \path[line] (1) edge[sloped] node[above]{$\aout[a][c][token]$} (2);
        \path[line] (1) edge[sloped] node[below]{$\aout[a][c][error]$} (3);
%
        \node[draw,text width=1.8cm] at (0.5,1) {$\ptp[A]$: Auth. server};
    \end{tikzpicture}
% \qquad
    \begin{tikzpicture}[node distance=1cm and 1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (0) {};
        \foreach \s/\t in {0/1,1/1b,1b/2,2/3,3/4,4/5,5/6} {
           \node (\t) [cnode, right = of \s] {};
        }
        \foreach \s/\l/\t in {0/\ain[c][s][helo]/1,1/\ain[s][c][token]/1b,1b/\aout[s][c][int]/2,2/\ain[c][s][read]/3,3/\aout[s][c][size]/4,4/\ain[c][s][retr]/5,5/\aout[s][c][msg]/6} {
           \path[line,sloped] (\s) edge node[below]{$\l$} (\t);
        }
        \node[cnode,above = of 0] (7) {};
        \node[cnode,right = of 7] (8) {};
        \node[cnode,below = of 1b] (9) {};
        %
        \path[line] (d) -- (0);
        \path[line] (6) edge[bend left=-35] node[below]{$\ain[c][s][ack]$} (2);
        \path[line] (0) edge node[left]{$\ain[c][s][quit]$} (7);
        \path[line] (2) edge node[left]{$\ain[c][s][quit]$} (7);
        \path[line] (4) edge[sloped] node[above]{$\ain[c][s][quit]$} (7);
        \path[line] (7) edge node[above]{$\aout[s][c][bye]$} (8);
        \path[line] (1b) edge node[below right]{$\aout[s][c][fail]$} (9);
%
        \node[draw,text width=1.8cm] at (6,1.2) {$\ptp[S]$: POP server};
    \end{tikzpicture}
\\
    \begin{tikzpicture}[node distance=1cm and 1.1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (auth0) {};
        \node[cnode,right= of auth0] (auth1) {};
        \node[cnode,right= of auth1] (0) {};
        \node[cnode,above= of auth1] (authFail) {};
%        
        \foreach \s/\t in {0/1,1/1b,1b/2,2/3,3/4,4/5,5/6} {
           \node (\t) [cnode, right = of \s] {};
        }
        \foreach \s/\l/\t in {0/\aout[c][s][helo]/1,1/\aout[c][s][token]/1b,1b/\ain[s][c][int]/2,2/\aout[c][s][read]/3,3/\ain[s][c][size]/4,4/\aout[c][s][retr]/5,5/\ain[s][c][msg]/6} {
           \path[line,sloped] (\s) edge node[below]{$\l$} (\t);
        }
        \node[cnode,above = of 0] (7) {};
        \node[cnode,right = of 7] (8) {};
        \node[cnode,below = of 1b] (9) {};
%        
        \path[line] (d) -- (auth0);
        \path[line] (auth0) edge node[below]{$\aout[c][a][cred]$} (auth1);
        \path[line] (auth1) edge node[left]{$\ain[a][c][error]$} (authFail);
        \path[line] (auth1) edge node[below]{$\ain[a][c][token]$} (0);
        \path[line] (6) edge[bend left=-35] node[below]{$\aout[c][s][ack]$} (2);
        \path[line] (0) edge node[left]{$\aout[c][s][quit]$} (7);
        \path[line] (2) edge node[left]{$\aout[c][s][quit]$} (7);
        \path[line] (4) edge[sloped] node[above]{$\aout[c][s][quit]$} (7);
        \path[line] (7) edge node[above]{$\ain[s][c][bye]$} (8);
        \path[line] (1b) edge node[below right]{$\ain[s][c][fail]$} (9);
%
        \node[draw,text width=1.8cm] at (0.5,1) {$\ptp[C]$: POP client};
    \end{tikzpicture}
    % \caption{Communicating system for POP with authentication}
\end{align*}
% In this case, since $\gpop{pop'}$ is well-formed,
% the machines are correct by construction.
% 
% Otherwise, we can use ChorGram to check multiparty
% compatibility~\cite{lange:gay17}, which indicates if the components
% will be able to interact successfully.
% %
% In such case, ChorGram also computes a g-choreography that
% faithfully represent the behaviour of the CFSMs.
% 

\noindent\textbf{Step \ref{it:qos}} The identification of QoS attributes and
the relative constraints, as well as the identification of final
states of CFSMs are application dependent tasks that requires human
intervention.
%
\aGcomm[Find existing SLAs in AWS catalogue and expand this]{If a
  component is to be realized by a service taken from an existing
  catalogue, as can be donde with the AWS cloud, then its QoS attributes
  and their constraints can be obtained from the service's
  SLA}. 

\noindent\textbf{Step \ref{it:qcfsm}}
This phase of our methodology assigns QoS constraints identified in
Step~\ref{it:qos} to specific states of the CFSMs determined in
Step~\ref{it:cfsm}.
%
This yields the set of qCFSMs of the systems.
%
\eMcomm[say  that \thetool supports this]{}
An example of a CFSM extended with QoS specifications for participant
\ptp[C] was shown in \cref{ex:pop-cfsm-qos}.
%
The QoS specifications for the other components are omitted for
brevity.
%
% As for POP, our  QoS attributes are time, monetary cost, and
% memory (together with the same aggregation operators used so far).
%
% The assignement of QoS specification to CFSMs is crucial; the quality
% of the analysis strongly depends on this step: the more accurate QoS
% specifications are the more accurate the results of the analysis will
% be.
%
% For the sake of the presentation, let
% $\Gamma_{\constset[Q]_{\mathrm{Chk}}} = \{ t \leq 5, c = 0.5, m = 0
% \}$ be one of our QoS specification. Following the rationale already 
% used in \cref{ex:qosspec}, $\Gamma_{\constset[Q]_{\mathrm{Chk}}}$ 
% models the computational costs of checking the integrity of a received
% message. Therefore it would be mapped to \p[c] right 
% after receiving a message, as the following fragment of the machine \p[c] shows:
% % \begin{center}
% \begin{align*}
%     \begin{tikzpicture}[node distance=1cm and 1.3cm, every node/.style={scale=1,transform shape}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
%         \def\chk{\Gamma_{\constset[Q]_{\mathrm{Chk}}}}
%         \node[cnode] (0) at (0,0) {};
%         \node[cnode, left= of 0] (-1) {};
%         \node[left= of -1] (-2) {};
%         \node[cnode,right= of 0, label=$\chk$] (1) {};
%         % \node[label={above:$\{ t \leq 5, m = 0 \}$}] (1) {$\aQzero$};
%         \node[right= of 1] (2) {};
% %
%         \path (-2) -- node[auto=false]{\ldots} (-1);
%         \path[line] (-1) edge node[below]{$\aout[c][s][retr]$} (0);
%         \path[line] (0) edge node[below]{$\ain[s][c][msg]$} (1);
%         \path (1) -- node[auto=false]{\ldots} (2);
%     \end{tikzpicture}
% \end{align*}
% % \end{center}
% If this procedure is repeated for every state in every machine then
%  we have a complete QoS-extended system, a comprehensive QoS aware 
%  model of the behaviour of the system.
% 
% The output of these steps is a \texttt{.qosfsa} file, containing the QoS-extended communicating system.

\noindent\textbf{Step~\ref{it:ql}} This phase shifts the focus to
specifying the properties of interest of the overall system.
%
The designer expresses this property in the QoS logic $\QL$.
% and written in a \texttt{.ql} file.
%
Suppose we would like to verify that a specific relation between the
monetary cost for the client $\p[c]$ to download messages and the
execution time holds. For instance, let $\psi$ be the constraint
$t > 1 \implies c < 10 t$ stating that, whenever the aggregated time
is above one second, the monetary cost is lower than ten times the aggregated
time.
%
The structure of our property is then as follows
$\gqosprop = [\aG] \psi$ (recall that $\gqosprop$
is equivivalent to
$\neg\ (\top\ \until[\aG]\ \neg\psi)$).
%
An essential part of the process of accurately defining $\gqosprop$ is to identify
the g-choreography $\aG$ that characterises the runs of the system
that we want to analyse.
%
We can determine $\aG$ by inspecting the g-choreography $\aG_{\mathsf{auth}}$
above, in order to identify the point(s) of the protocol where \p[c] downloads
messages; \aGcomm[check g-chor]{this yields}
\begin{align*}
  \aG = &\ \gint[][c][cred][a];
			 \gint[][a][token][c];
			 \gint[][c][helo][s];
			 \gint[][c][token][s];
			 \gint[][s][int][c];
			 \grec[][\aG_1]
\end{align*}
where
$\aG_1 = \gint[][c][read][s]; \gint[][s][size][c];
\gint[][c][retr][s]; \gint[][s][msg][c]; \gint[][c][ack][s]$.
%
In words, $\aG$ above characterises runs where, after successful
authentication, \p[c] iteratively downloads messages from \p[s].

\noindent\textbf{Step~\ref{it:mc}} The last step of our methodology
consists in verifying the QoS property $\gqosprop$.
%
We can check whether there is a run in the QoS extended communicating
system that satisfies the QoS property $\gqosprop$.
%
\eMcomm[summarise the rest without the technicalitieis]{This verification is fully supported by our tool.}
%
\hsl[all this and the stuff I commented above goes in the artefact submission]
, by the by calling
\thetool using the following command:

\begin{center}
\begin{minipage}{.8\linewidth}
\begin{lstlisting}[style=ql, basicstyle=\ttfamily\footnotesize, numbers=none]
    mocheqos satisfiability sys.qosfsa prop.ql <k>
\end{lstlisting}
\end{minipage}
\end{center}%
where \texttt{<k>} specifies the bound on the length of the runs to be considered.
A natural choice for our scenario is to derive $k$ from fixing an upper bound on
the number of messages received by $\p[c]$, that is on the number of iterations of $\aG_1$ in $\aG$.
% 
Instead, if we are interested in checking if the property is valid, that is if it holds for all runs of the system, we can use the following command:
\begin{center}
\begin{minipage}{.8\linewidth}
\begin{lstlisting}[style=ql, basicstyle=\ttfamily\footnotesize, numbers=none]
    mocheqos validity sys.qosfsa prop.ql <k>
\end{lstlisting}
\end{minipage}
\end{center}
Again, \texttt{<k>} specifies the bound on the length of the runs to be considered. 
The analysis in this case is essentially a counterexample finding procedure.
If no counterexample is found, then we have the guarantee that the property holds for all runs of the system, up to the bound $k$.
At such point, we might choose to increase the bound $k$ and repeat the procedure in order to have guarantees for larger numbers of iterations of the g-choreography.
If, on the other hand, the property is violated within the bound $k$, \thetool will return a counterexample, that is a run of the system that serves as a witness of such a violation. This allows the designer to identify the source of the violation and to take appropriate actions.
% Formula $\gqosprop$ can be verified with a bounded model checking approach
% (cf. \cref{sec:analysis}).
% %
% This approach requires to first choose a bound $k$ for the number of
% iterations in $\aG$ in order to obtain a formula $\gqosprop'$ in $\QL^-$.
% %
% %
% Then, we can feed \textsc{qSat} with the formula $\neg\gqosprop'$,
% together with the QoS extended communicating system. The analysis will
% tell whether $\neg\gqosprop'$ is satisfiable or not. If
% $\neg\gqosprop'$ is not satisfiable we have the guarantee that every
% run of the system, up to $k$ messages received by $\p[c]$, satisfies
% the formula $\gqosprop$. 
% 
% At this point we might choose to increase the
% bound $k$ and repeat the procedure in order to have guarantees for
% larger numbers of iterations of the g-choreography. If, on the other
% hand, $\neg\gqosprop'$ is satisfiable, we can be certain that the
% system violates formula $\gqosprop$ because there exists an execution
% that serves as a witness of such a violation.  Finally, after that
% verdict, there are different possible courses of action.  We might
% weaken the QoS constraint $\psi$ in order to check a looser constraint
% or we might modify the QoS specifications assigned to the states of
% the components of the systems, aiming at strengthening them in order
% to satisfy $\gqosprop$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> old_aws.tex <==
In order to test for the applicability of the technique we will conduct experiments on systems of two different natures. 
%
In the first place, we develop a case study within the AWS Cloud infrastructure. In AWS Cloud, the pricing scheme is, generally, pay as you go on a monthly basis and it is determined by values assigned to a specific list of attributes. These attributes make the pricing scheme parametric and can be classified in:
\begin{itemize}
\item cumulative, like storage (provided by the AWS Elastic Block Storage service\footnote{Documentation available at \url{https://aws.amazon.com/ebs/}.}), measured in Gb and paid per month of provisioned storage and, computation (provided by the AWS Elastic Compute Capacity service\footnote{Documentation available at \url{https://aws.amazon.com/ec2/}.}) and software execution, both paid per hours of compute time, and
\item non-cumulative, like region and fulfillment option, both ranging over a finite list of possible values, and impacting on the unitary values paid for the cumulative 
\end{itemize}
In addition to the parametric pricing scheme mentioned above, the selection of a specific server configuration for deploying the service, being this another non-cumulative attribute, have a direct impact on other quantitative attributes of interest, like, for example, the transfer rate, which, in turn, impact the final price that will be paid in a given month.

In principle, there are two obstacles for interpreting AWS’ SLAs within the contracts in~\cite{lopezpombo:ictac23}. On the one hand, there is a granularity mismatch between AWS’s SLAs (i.e., the pricing scheme) and the more structured view of process presented in our work. While AWS’s SLAs can be considered monolithic, our automata-based language formalizes components as a composition of tasks represented by the nodes, expressing computations and communication interaction represented by the arrows. This way of describing the behavior of participants provide a more fine-grain view of how the service is executed allowing also a compositional understanding of the costs involved in it. On the other hand, while it is very easy to model the price as the result of accumulating the base values per time/storage unit, multiplied by the time/space required, scaled by the transfer rate, it is important to consider that non-cumulative attributes, which determine the base values, are not directly representable in our approach because attributes are always interpreted as real.

For the sake of showing the potential behind our proposal we will take the SLAs available at AWS marketplace and feature a version of it but compatible with the formal language proposed in our work; in addition, we will represent non-cumulative attributes by building a bijection between the discrete choices in the list and natural numbers. Then, the specification of all the possible configuration can be modeled by a collection of formulae with the shape ``$\left( \bigwedge [ \mathit{non\_cummulative\_attr} ] = [ \mathit{natural\_number} ] \right) \implies \left( \bigwedge [ \mathit{attr} ] = [ \mathit{value} ] \right)$'' therefore, choosing a specific configuration for the service pricing scheme from the available ones boils down to assigning a combination of natural numbers to the corresponding non-cumulative attributes determining the configuration. 

%%%%%

Secondly, we will evaluate the technique over communicating systems
automatically extracted from code. In~\cite{imai:tacas22}, Imai et. al. 
presented a library capable of verifying the compatibility of concurrent
message-passing programs.
%
This library features a type inference algorithm that extracts CFSMs
directly from OCaml code.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pop.tex <==
Through the paper we will use a (simplified variant) of the POP
protocol~\cite{rfc937}.
%
This protocol allows mail clients to access a remote mailbox and
retrieve e-mails.
%
In the POP protocol a client starts the communication by sending a
message of type $\msg[helo]$ to a POP server (note that protocol
specifications are oblivious of messages' payload).\footnote{Our
  framework can handle multiparty protocols; however, our examples are
  two-party for simplicity. Also, we stick to the types of messages as
  carefully described in the protocol specifications~\cite{rfc937}.  }
%
%
The server replies with the number of unread messages in the mailbox
using a message of type $\msg[int]$.
%
At this point the client can either halt the protocol or
read one of the e-mails.
%
These options are selected by sending a message of type $\msg[quit]$
or of type $\msg[read]$ respectively.
%
In the former case, the server acknowledges with a message of type
$\msg[bye]$ and the protocol ends.
%
In the latter case, the server sends the client the number of bytes of
the current unread message in a message of type $\msg[size]$.
%
Next, the client has again a choice between quitting the protocol (as
before) or receiving the email (selected in the $\msg[read]$ message)
by sending the server a message of type $\msg[retr]$.
%
In the latter case the server sends the email with a message of type
$\msg[msg]$, the client answers with a message of type $\msg[ack]$
and the reading process starts again.

%
% However, in \cref{sec:methodology} we will consider a multi-party
% variant of the POP protocol where the client has first to provide the
% POP server with an authentication token received by a third-party
% server.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> qoschoreo.tex <==
% !TEX root = ./main.tex

In this section we extend CFSMs with QoS specifications in order to
express QoS contracts of components in message-passing systems.
%
Basically, each state of CFSMs is assigned a QoS contract specifying
the usage of computational resources.
%
We formalise QoS contracts as \emph{QoS specifications}
which are theory presentations over the
RCFs, noted as $\conf{\Sigma, \Gamma}$, paired up with \emph{aggregation operators}, noted as $\oplus^\genericAttr$,
to define how each
QoS attribute accumulates along a communicating system. 
These aggregation operators will be essential to formally define the notion of aggregation along a run, as shown later in \cref{ex:aggregation-function}.
%
\begin{definition}\label{def:qos-spec}
  A \emph{QoS specification} $\conf{\Sigma, \Gamma}$ is a
  (first-order) theory presentation extending
  $\conf{\Sigma_\mathrm{RCF}, \Gamma_\mathrm{RCF}}$ as follows:
  \begin{enumerate}
  \item
	 $\Sigma = \conf{\{0, 1\} \cup \constset[Q], \{+, \cdot\} \cup
		\{\oplus^\genericAttr\}_{\genericAttr \in \constset[Q]}, \{<\}}$, where $\constset[Q]$
	 is a finite set of constant symbols (other that
	 $0$ and $1$) representing the \emph{quantitative attributes} (from
	 now on referred to as \emph{QoS attributes}) and, for each
	 $\genericAttr \in \constset[Q]$, $\oplus^\genericAttr$ is an associative
	 algebraic binary operator 
  %  (cf. \cref{def:algop} in
	%  \cref{sec:aux}) 
   and
  \item $\Gamma = \Gamma_\mathrm{RCF} \cup \text{$\Gamma^\prime$}$,
	 being $\Gamma^\prime$ a finite set of
	 first-order formulae formalising specific constraints over 
   the QoS attributes in $\constset[Q]$.
  \end{enumerate}
  % 
  The class of QoS specifications will be denoted as $\qosspecs(\constset[Q])$.
\end{definition}
%
In order to preserve decidability of QoS properties, we only consider
QoS specifications involving additional constant symbols representing
the QoS attributes of components.
%
Aggregation operators are required to be algebraic %(\cref{sec:aux})
because the extension of the theory must be kept in the first-order
fragment (uninterpreted function or predicate symbols must be avoided
to preserve decidability).
%
It is worth noticing that aggregation operators strongly depend on the
nature of each specific attribute; for example, natural aggregation
operators for memory and time are the maximum function and sum respectively.

\begin{example}[QoS specification]\label{ex:qosspec-detailed}
  With reference to \cref{ex:pop}, possible quantitative attributes of
  interest in an implementation of POP are
  $\constset[Q]=\{t, c, m\}$ representing CPU \textit{t}ime, monetary \textit{c}ost, 
  and \textit{m}emory usage, respectively.
  %
  Then a QoS specification that characterises low computational
  costs, where no internal process consumes significant amount of
  resources, can be written according to \cref{def:qos-spec} as follows:
  \begin{align*}
    \Sigma = &\ \conf{\{0, 1\} \cup \{t, c, m\}, \{+, \cdot\} \cup
     \{\oplus^t, \oplus^c, \oplus^m\}, \{<\}} \\
            % 
   \Gamma = &\ \Gamma_\mathrm{RCF} \cup \Gamma^\prime_\mathrm{Low}
            % & 
  \end{align*}%
  where $\oplus^t = +,\ \oplus^c = +,\ \oplus^m = \mathit{max}$, and
  $\Gamma^\prime_\mathrm{Low} = \{t \leq .01, c \leq .01, m \leq .01\}$
  \finex
\end{example}

From now on, we fix a set of constant symbols $\constset[Q]$ which we
omit from the set of \emph{QoS specifications}, that will be referred
to just as $\qosspecs$.  It is worth noting that, when $\constset[Q]$
is fixed, a QoS specification
$\conf{\Sigma, \Gamma_\mathrm{RCF} \cup \Gamma^\prime}$, is
  completely determined by $\Gamma^\prime$.
  %
  Therefore, we can unabiguously refer
  to % will employ an abuse of notation, defining
  a QoS specification using its set of formulas $\Gamma^\prime$.
  Thus, the QoS specification in \cref{ex:qosspec-detailed}
is $\Gamma^\prime_\mathrm{Low}$.
\begin{example}[QoS for POP]\label{ex:qosspec}
The following QoS specifications formalise the costs associated to different
activities in the POP protocol of \cref{ex:pop}.
  \begin{align*}
    % & \Gamma_\mathrm{Low} = \{t \leq 0.01, c \leq 0.01, m \leq 0.01\} \qquad\qquad
    & \Gamma^\prime_\mathrm{Chk} = \{ t \leq 5, c = 0.5, m = 0 \} \\
    & \Gamma^\prime_\mathrm{Mem} = \{ 1 \leq t \leq 6, c = 0, m \leq 64 \} \\
    & \Gamma^\prime_\mathrm{DB} = \{ t \leq 3 \implies (\exists x)(0.5 \leq x \leq 1 \land c = t \cdot x),
                                            t > 3 \implies c = 10,
                                            m \leq 5 \}
  \end{align*}
  Basically, $\Gamma^\prime_\mathrm{Chk}$
  formalizes the costs associated to the activity of
  integrity checking a message,
  $\Gamma^\prime_\mathrm{Mem}$ to the activity of a server
  receiving a message, and $\Gamma^\prime_\mathrm{DB}$ to
  establishing that the monetary cost is fixed if the insertion takes
  more than three time-units and it is a fraction of the
  execution time, otherwise.
  % 
  \finex
\end{example}
 
We now extend communicating systems (cf. \cref{sec:pre}) with
QoS-specifications.
%
\begin{definition}[QoS-extended CFSMs]\label{def:cfsm-extend}%
  A \emph{QoS-extended CFSM} is a tuple
  $\aCMq = \conf{\aCM, F, \qos}$ where:
  \begin{itemize}
  \item $\aCM = \conf{Q, q_0, \rightarrow }$ is a CFSM,
  \item $F \subseteq Q$ is a set of \emph{final states} of $\aCM$, and
  \item $\qos: Q \to \qosspecs$ maps states of $\aCM$ to QoS
	 specifications.
 \end{itemize}
 A \emph{QoS-extended communicating system} $S^{\mathit{QoS}}$ is a
 map $(\aCMq_{\p})_{\p \in \PSet}$ assigning an $\p$-local
 QoS-extended CFSM $\aCMq_{\p}$ to each $\p \in \PSet$.  A
 configuration $\csconf q \abuffer$ of $S^{\mathit{QoS}}$ is a
 \emph{final configuration} if $\vec q(\p) \in F_{\p}$ for every
 $\p \in \PSet$.
 % , and the signature $\Sigma$ is the same among all machines.
\end{definition}

\begin{example}[QoS-extended CFSMs] 
  %
  \label{ex:pop-cfsm-qos}
  An extended CFSM of the POP client in \cref{ex:pop} with the QoS
  specifications of \cref{ex:qosspec} is as follows:
  %
%  \begin{figure}[ht]
%    \centering
  \begin{center}
%    \includegraphics[width=0.8\textwidth,valign=c]{ex-pop-qos.pdf}
  \begin{tikzpicture}[node distance=1cm and 1.3cm, every node/.style={scale=1,transform shape}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
	 \def\low{\Gamma^\prime_\mathrm{Low}}
	 \def\db{\Gamma^\prime_\mathrm{DB}}
	 \def\mem{\Gamma^\prime_\mathrm{Mem}}
	 \def\chk{\Gamma^\prime_\mathrm{Chk}}
	 \node (d) at (0,0) {};
	 \node[cnode,right= .3cm of d, label={-95:$\low$}] (0) {};
	 \foreach \s/\l/\t in {0/\low/1,1/\db/2,2/\low/3,3/\db/4,4/\mem/5,5/\chk/6} {
		\node (\t) [cnode, right = of \s, label={$\l$}] {};
	 }
	 \foreach \s/\l/\t in {0/\aout[c][s][helo]/1,1/\ain[s][c][int]/2,2/\aout[c][s][read]/3,3/\ain[s][c][size]/4,4/\aout[c][s][retr]/5,5/\ain[s][c][msg]/6} {
		\path[line,sloped] (\s) edge node[below]{$\l$} (\t);
	 }
	 \node[cnode, above = of 0, label={95:$\low$}] (7) {};
	 \node[cnode, right = of 7, label={10:$\low$}, fill = black] (8) {};
	 %
	 \path[line] (d) -- (0);
	 \path[line] (6) edge[bend left=-35] node[below]{$\aout[c][s][ack]$} (2);
	 \path[line] (0) edge node[left]{$\aout[c][s][quit]$} (7);
	 \path[line] (2) edge[sloped] node[below,near end]{$\aout[c][s][quit]$} (7);
	 \path[line] (4) edge[sloped] node[above]{$\aout[c][s][quit]$} (7);
	 \path[line] (7) edge node[above]{$\ain[s][c][bye]$} (8);
  \end{tikzpicture}
  \end{center}
  where the filled state is the only final state.
  % \eMcomm[remove?]{The CFSM of the server could be extended in a similar way.}
  % 
%    \caption{QoS-extended CFSM of a \textit{Client} in the simplified POP protocol.}\label{fig:ex-pop-qos}
%  \end{figure}
  %
  Each state is assigned a QoS specification given in
  \cref{ex:qosspec} according to the following idea.
  %
  States where the client performs negligible computations are
  assigned the QoS specification
  $\Gamma^\prime_\mathrm{Low}$.
  %
  The remaining states are assigned QoS specifications as follows.
  % \begin{itemize}[label=-]
  % \item
  The local states where \p[c] performs a database insertion (right
  after receiving an $\msg[int]$ or $\msg[size]$ message) and those
  where \p[c] accesses the memory (right before receiving an unread
  e-mail) are constrained respectively by $\Gamma^\prime_\mathrm{DB}$
  and $\Gamma^\prime_\mathrm{Mem}$; finally,
  % \item
   $\Gamma^\prime_\mathrm{Chk}$ constrains the states where \p[c]
	performs an integrity check (right after receiving an unread
	e-mail).
  % \end{itemize}
  % For example, the assignment of QoS specifications to the states of
  % the CFSM of \cref{ex:pop} specifies (as mentioned in
  % \cref{ex:qosspec}) that in the initial state does not consume a
  % significant amount of resources.
  %  
  \finex
\end{example}

Notice that \cref{def:cfsm-extend} requires every
  state of a CFSM to be assigned a QoS specification. However, in most
  cases, most states will have the same QoS specification, as it is the
  case of $\Gamma^\prime_\mathrm{Low}$ in
\cref{ex:pop-cfsm-qos}; typically one only has to
  identify the QoS costs specific to few states.

The semantics of QoS-extended communicating systems is defined in the
same way as the semantics of communicating systems. This is a
consequence of the fact that QoS specifications do not have any effect
on communications.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> qsat.tex <==
\begin{algorithm}[H]
% \caption{Decision procedure for the satisfiability of $\QL^-$ formulae}
% \label{alg:check}
\DontPrintSemicolon
\SetAlgoLined
\KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
\KwResult{A set of runs: $\emptyset \iff \aCS \models \gqosprop$}
\SetKwFunction{check}{\textsc{qSat}}
\SetKwFunction{traceOf}{\textsc{TraceOf}}
\check{$\gqosprop,\aCS,\pi$}:\\
\lnl{1}\lIf{$\gqosprop \in \qosspecs$}{
  \Switch{\texttt{SMT}($\aggfn (\pi), \gqosprop$)}{
	 \lCase{\textbf{true}}{\Return{$\emptyset$}}
    \lCase{\textbf{false}}{\Return{$\{\pi\}$}}
  }
}
\Switch{$\gqosprop$}{
  \lnl{2}\lCase{$\neg\gqospropb$}{
	 \Switch{$\gqospropb,\aCS,\pi$}{
		\lCase{$\emptyset$}{\Return{$\{\pi\}$}}
		\lCase{\textbf{otherwise}}{\Return{$\emptyset$}}
	 }
  }
  \lnl{3}\lCase{$\gqospropb \lor \gqospropb'$}{
	 \Switch{\check{$\gqospropb,\aCS,\pi$}}{
		\lCase{$\emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
		\lCase{\textbf{otherwise}}{\Return{$\{\pi\}$}}
	 }
  }
  \Case{$\gqospropb\ \qluntil\ \gqospropb'$}{
	 \lnl{4}\lIf{\check{$\gqospropb',\aCS,\pi$} == $\emptyset$}{\Return{$\emptyset$}}
	 \Else{
		\lnl{5}\ForEach{$\aConf \TRANSS{\al} \aConf'$ on $\aCS$}{
		  \lnl{6}\lIf{\check{$\gqospropb,\aCS,\pi$} == $\emptyset$
			 \textbf{\emph{and}}
			 \traceOf{$\pi \cdot \aConf \TRANSS{\al} \aConf'$}
			 $\in \mathcal{L}(\aG)$}{
			 \check{$\gqospropb\ \qluntil\ \gqospropb',\aCS, \pi \cdot \aConf \TRANSS{\al} \aConf'$}}
		}
	 }
  }
  \lnl{8}\lCase{$\top$}{\Return{$\emptyset$}}
  \lnl{9}\lCase{$\bot$}{\Return{$\{\pi\}$}}
}
\end{algorithm}


\begin{algorithm}[H]
% \caption{Decision procedure for the satisfiability of $\QL^-$ formulae}
% \label{alg:check}
\DontPrintSemicolon
\SetAlgoLined
\KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
\KwResult{A singleton with a witness that $\aCS\models \gqosprop$ (if any, otherwise $\emptyset$)}
\SetKwFunction{check}{\textsc{qSat}}
\SetKwFunction{traceOf}{\textsc{TraceOf}}
\check{$\gqosprop,\aCS,\pi$}:\\
\lnl{1}\lIf{$\gqosprop \in \qosspecs$}{
  \Switch{\texttt{SMT}($\aggfn (\pi), \gqosprop$)}{
	 \lCase{\textbf{true}}{\Return{$\{\pi\}$}}
    \lCase{\textbf{false}}{\Return{$\emptyset$}}
  }
}
\Switch{$\gqosprop$}{
  \lnl{2}\lCase{$\neg\gqospropb$}{
	 let tmp = \check{$\gqospropb,\aCS,\pi$} 
	 \Switch{tmp}{
		\lCase{$\emptyset$}{\Return{$\{\pi\}$}}
		\lCase{\textbf{otherwise}}{\Return{$\emptyset$}}
	 }
  }
  \lnl{3}\lCase{$\gqospropb \lor \gqospropb'$}{
	 let tmp = {\check{$\gqospropb,\aCS,\pi$}}
	 \Switch{tmp}{
		\lCase{$\emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
		\lCase{\textbf{otherwise}}{\Return{tmp}}
	 }
  }
  \Case{$\gqospropb\ \qluntil\ \gqospropb'$}{
	 \lnl{4}\lIf{\check{$\gqospropb',\aCS,\pi$} $\neq \emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
	 \Else{
		\lnl{5}\ForEach{$\aConf \TRANSS{\al} \aConf'$ on $\aCS$}{
		  \lnl{6}\lIf{{\check{$\gqospropb,\aCS,\pi$}} $\neq \emptyset$
  \textbf{\emph{and}}
			 \traceOf{$\pi \cdot \aConf \TRANSS{\al} \aConf'$}			 $\in \mathcal{L}(\aG)$
}{	 let tmp = 			 \check{$\gqospropb\ \qluntil\ \gqospropb',\aCS, \pi \cdot \aConf \TRANSS{\al} \aConf'$}
			 \lIf{\\tmp \neq $\emptyset$}{\Return{tmp}}
}{
		  }
		}
	 }
  }
  \lnl{8}\lCase{$\top$}{\Return{$\{\pi\}$}}
  \lnl{9}\lCase{$\bot$}{\Return{$\emptyset$}}
}
\end{algorithm}
\end{document}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rcf.tex <==
%!TEX root = ./main.tex
%c
% Real numbers are natural candidates to express quantitative attributes
% of a software artefact.
% %
% We adopt \emph{real-closed fields} (RCFs), the formalisation of the
% first-order theory of the real numbers, as a foundations for QoS
% values.
% %
% The main reason for this choice is that theories extending the RCFs
% are decidable, providing effective means for analysis.
%
Hereafter, we assume that the reader is acquainted with the
language of first-order predicate logic with equality
($\mathit{FOL}_=$), its semantics and associated
calculus~\cite{smullyan68,enderton72}.
%
We fix a denumerable set of variable symbols $\varset$ and an arbitrary
signature $\Sigma = \conf{\constset, \mathtt{F}, \mathtt{P}}$
consisting of the constant, function, and predicate symbols.
%
A first-order logic over $\Sigma$ is defined as usual.
%
Let $\termalg$ and $\formulas$ respectively denote the set of terms
and formulae over $\Sigma$ and $\varset$.

A \emph{$\Sigma$-interpretation} is a structure
$\mathcal{I} = \conf{S, \{\overline{c}\}_{c \in \constset},
  \{\overline{f}\}_{f \in \mathtt{F}}, \{\overline{p}\}_{p \in
	 \mathtt{P}}}$ assigning meaning to the symbols in $\Sigma$
respectively as elements of the \emph{carrier set} $S$, as functions,
and as predicates over $S$.
%
A \emph{model} $\mathcal{M}$ consists of a pair
$\conf{\mathcal{I}, v}$ where $\mathcal{I}$ is a
$\Sigma$-interpretation and $v: \varset \to S$ is a \emph{valuation}
assigning meaning to variables over the carrier set of
$\mathcal{I}$.
%
We let $\modelsclass$ to be the class of models for $\Sigma$,
$\varset$ and $\models \subseteq \modelsclass \times \formulas$ the
satisfaction relation recursively defined on the structure of the
formula as usual.
%
The entailment relation
$\vdash \subseteq 2^{\formulas} \times \formulas$ can be formalised
through axioms and rules
% as any complete calculus of choice
(see e.g.,~\cite{hilbert50}, \cite[Sec.~II]{gentzen:apq-1_4}, or \cite[Sec.~2.4]{enderton72}).
%
%Fixed an arbitrary signature $\Sigma = \conf{\constset, \mathtt{F}, \mathtt{P}}$ consisting of the constant, function, and predicate symbols and given a denumerable set of variable symbols $\varset$, an first-order logic over $\Sigma$ is defined as usual; let $\termalg$ and $\formulas$ to respectively be the set of terms and formulae over $\Sigma$ and $\varset$.
%
%A \emph{$\Sigma$-interpretation} is a structure $\mathcal{I} = \conf{S, \{\overline{c}\}_{c \in \constset}, \{\overline{f}\}_{f \in \mathtt{F}}, \{\overline{p}\}_{p \in \mathtt{P}}}$, where the set $S$ is the \emph{carrier set} such that:
%\begin{inparaenum}[i)] 
%\item $\overline{c} \in S$, for all $c \in \constset$, 
%\item $\overline{f}: S^{\mathit{arity(f)}} \to S$, for all $f \in \mathtt{F}$, and
%\item $\overline{p} \subseteq S^{\mathit{arity(p)}}$ for all $p \in \mathtt{P}$,
%\end{inparaenum}
%assigning meaning to the symbols as elements, functions and predicates over $S$, respectively.
%
%Given a signature $\Sigma$, a \emph{model} $\mathcal{M}$ consists of a
%pair $\conf{\mathcal{I}, v}$ where $\mathcal{I}$ is a
%$\Sigma$-interpretation and $v: \varset \to S$ is a \emph{valuation}
%assigning meaning to variables over the carrier set $S$ of
%$\mathcal{I}$.
%
%The class of models for $\Sigma, \varset$ is denoted as $\modelsclass$.
%
%The satisfaction relation between models and formulae $\models \subseteq \modelsclass \times \formulas$ is defined recursively on the structure of the formula as usual.
%
%The entailment relation $\vdash \subseteq 2^{\formulas} \times \formulas$ can be formalised through the axioms and rules of any complete calculus of choice (see, for instance, \cite[Drittes Kapitel]{hilbert28} for a Hilbert-style calculus, \cite[Sec.~II]{gentzen:apq-1_4} for a natural deduction calculus and \cite[Sec.~2.4]{enderton72} for a classical calculus, among others, and \cite{troelstra96} for a more comprehensive presentation of them).
%
A set of formulae $\Gamma \in 2^{\formulas}$ is a \emph{first-order theory} if
$\Gamma$ is closed under deduction (i.e., $\Gamma \vdash \alpha$
implies $\alpha \in \Gamma$ for all $\alpha \in \formulas$).
%
A \emph{(first-order) theory presentation over $\Sigma$} is a pair
$\conf{\Sigma, \Gamma}$ where $\Gamma \subseteq \formulas$.
%
The notion of model extends naturally to theory presentations:
$\mathcal{M} \models \conf{\Sigma, \Gamma}$ iff
$\mathcal{M} \in \modelsclass$ and $\mathcal{M} \models \varphi$, for
all $\varphi \in \Gamma$.

Let $\Sigma_{\mathrm{field}}$ be the signature $\conf{\{0, 1\},\{+, \cdot\},\{=\}}$.
%
An ordered field is a first-order theory presentation
$\conf{\Sigma_{\mathrm{field}}, \Gamma_{\mathrm{field}}}$ where
$\Gamma_{\mathrm{field}}$ are the field axioms 
% (cf.~\cref{def:ofield}
% in \cref{sec:auxrcf}).
%
Real-closed fields are ordered fields whose non-empty subsets all have
a supremum.% (cf.~\cref{def:RCF} in \cref{sec:auxrcf}).
%
In \cite{tarski:RM-109}, Tarski introduced \emph{the system of
  elementary algebra} as a first-order theory of real numbers for
which he proved that:
\begin{inparaenum}[a)]
\item it is a real-closed field \cite[Note~15]{tarski:RM-109}, and
\item there exists a decision procedure \cite[Thm.~37]{tarski:RM-109}.
\end{inparaenum}
Furthermore, all real-closed fields are isomorphic
\cite{erdos:am-3_61}(Thm.~2.1). 
% See \cref{sec:auxrcf} for a more
% detailed account on the theoretical aspects of the real-closed
% fields.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sem.tex <==
\anote{Review integration of text, examples and formal definitions in this section.}

The semantics of g-choreographies has been defined in
\cite{tuosto:jlamp-95} in terms of \emph{pomsets}
\cite{pratt:ijpp-15_1} labelled over
the set of \emph{communication actions}
$\lset = \lset^!  \cup \lset^?$.


Basically, the semantics $\gsem$ of a g-choreography $\aG$ is a set of
pomsets representing the causal relations among communication events
in $\aG$.
%
Due to space limitations, we give only an intuitive account of the
semantics 
% (
	% a compact technical presentation is in
% \cref{sec:sem}; 
(the reader is referred
to~\cite{tuosto:jlamp-95} for more details).
%
For instance, the semantics of an interaction is just a partial order
such that the event corresponding to the output precedes the one
corresponding to the input while the semantics of a parallel $\gpar[]$
composition is obtained by taking the disjoint unions of each pomset
in $\gsem$ and each one in $\gsem[\aG']$.
%
It is a straightforward observation that the semantics of $\star$-free
g-choreographies is a finite disjoint union of finite pomset.
%
We illustrate this intuition in the next example.
%
\begin{example}[An excerpt of POP's semantics]\label{ex:sem}
  The semantics of $\gpop{quit}$ in~\cref{ex:gpop} and of
  $\aG = \gint[][c][helo][s]; \gint[][s][int][c]$ (representing a
  possible initial run of POP) are the singletons
  \begin{align*}
	 \begin{array}[c]{c@{\qqand}c}
		\gsem[\gpop{quit}] = \left\{\pomset[1]{
		\node (1) {$\aout[c][s][quit]$};
		\node[right = of 1] (2) {$\ain[c][s][quit]$};
		\node[below = of 1] (3) {$\ain[s][c][bye]$};
		\node[below = of 2] (4) {$\aout[s][c][bye]$};
		%
		\path[draw,->] (1) -- (2);
		\path[draw,->] (4) -- (3);
		\path[draw,->] (1) -- (3);
		\path[draw,->] (2) -- (4);
		}
		\right\}
		&
		\gsem = \left\{\pomset[1]{
		\node (1) {$\aout[c][s][helo]$};
		\node[right = of 1] (2) {$\ain[c][s][helo]$};
		\node[below = of 1] (3) {$\ain[s][c][int]$};
		\node[below = of 2] (4) {$\aout[s][c][int]$};
		%
		\path[draw,->] (1) -- (2);
		\path[draw,->] (4) -- (3);
		\path[draw,->] (1) -- (3);
		\path[draw,->] (2) -- (4);
		}
		\right\}
	 \end{array}
  \end{align*}
  where we represent pomsets as (a variant\footnote{Edges of Hasse
	 diagrams are usually not oriented; here we use arrows so to draw
	 order relations between events also horizontally.} of) Hasse
  diagrams of the immediate predecessor relation enclosed in square
  brackets.\anote{R2: ‘Hasse diagrams of the immediate predecessor relation’ - please explain more, this sentence requires some background notion that is out of context here.}
  %
  Accordingly, we have $\gsem[{\gcho[][\gpop{quit}][\aG]}] = \gsem[\gpop{quit}] \cup \gsem[\aG]$
  while
  \begin{align*}
	 \gsem[{\gpar[][\gpop{quit}][\aG]}] =
	 \left\{\pomset[1]{
	 \node (1) {$\aout[c][s][helo]$};
	 \node[right = of 1] (2) {$\ain[c][s][helo]$};
	 \node[below = of 1] (3) {$\ain[s][c][int]$};
	 \node[below = of 2] (4) {$\aout[s][c][int]$};
	 %
	 \path[draw,->] (1) -- (2);
	 \path[draw,->] (4) -- (3);
	 \path[draw,->] (1) -- (3);
	 \path[draw,->] (2) -- (4);
	 %%
	 \node[right = 1cm of 2] (a) {$\aout[c][s][quit]$};
	 \node[right = of a] (b) {$\ain[c][s][quit]$};
	 \node[below = of a] (c) {$\ain[s][c][bye]$};
	 \node[below = of b] (d) {$\aout[s][c][bye]$};
	 %
	 \path[draw,->] (a) -- (b);
	 \path[draw,->] (d) -- (c);
	 \path[draw,->] (a) -- (c);
	 \path[draw,->] (b) -- (d);
	 }
	 \right\}
  \end{align*}
  formalising that the communications in $\gpop{quit}$ and those in
  $\aG$ may occur in any order since they are not related by any
  causal dependency.
  %
  \finex
\end{example}

The \emph{linearisations} of a pomset $\apom$ is the sequence of the communication
action obtained by a permutation of the events of $\apom$ that
preserves the causality relation of $\apom$.
%
For instance, the only possible linearisation of the pomset in
$\gsem[\gpop{quit}]$ (cf. \cref{ex:sem}) is the sequence
$\aout[c][s][quit]\ \ain[c][s][quit]\ \aout[s][c][bye]\
\ain[s][c][bye]$ while
$\aout[c][s][quit]\ \aout[s][c][bye]\ \ain[c][s][quit]\
\ain[s][c][bye]$ is not a linearisation because it violates the causal
dependency between $\aout[s][c][bye]$ and $\ain[c][s][quit]$.
%
The \emph{language} of $\aG$ is the set $\rlang[\aG]$ of sequences of
linearisations of a pomsets in $\gsem$.

\begin{definition}
  A labelled partially-ordered set (lposet) is a triple
  $(\eset, \leq, \alf)$, with $\eset$ a set of events,
  $\leq \subseteq \eset \times \eset$ a reflexive, anti-symmetric, and
  transitive relation on $\eset$, and $\alf: \eset \rightarrow \lset$ a
  labelling function.
\end{definition}
For $\ae \neq \ae'$, $\alf(\ae) = \alf(\ae')$ means that $\ae$ and $\ae'$
 model different occurrences of the same action.
Intuitively, $\leq$ represents causality;
for $\ae \neq \ae'$, if $\ae \leq \ae'$
and both events occur then $\ae'$ is
caused by $\ae$.
%
In the following, we use $\emptypom$ to denote the empty lposet and
$\ae \rightarrow \ae'$ to denote that $\ae \leq \ae'$.

\begin{definition}
  Two lposets $(\eset, \leq, \alf)$ and $(\eset', \leq', \alf')$ are
  isomorphic iff there exists a bijection
  $\phi: \eset \rightarrow \eset'$ such that $\ae \leq \ae'$ iff
  $\phi(\ae) \leq' \phi(\ae')$ and $\alf = \alf' \circ \phi$.
\end{definition}

\begin{definition}
  A partially-ordered multi-set (of actions), pomset for short, is an
  isomorphism class of lposets.
\end{definition}
%
In the following, $[\eset, \leq, \alf]$ denotes the isomorphism class
of $(\eset, \leq, \alf)$, we let $\apom,\apom', \dots$ (resp.
$\aR, \aR', \dots$) range over pomsets (resp. sets of pomsets), and we
assume that any $\apom$ contains at least one lposet which will
possibly be referred to as $(\esetof \apom$,
$\leqof \apom, \alfof \apom)$.

In the following, given a natural number $n$,
$\singleton{n}$ represents the singleton $\{n\}$.
%
Also, we use $X
\uplus Y$ to represent the disjoint union of two sets $X$ and $Y$: $X
\uplus Y = (X \times \singleton{1}) \cup (Y \times \singleton{2})$.
%
Finally, given a function $f$
on $X$,
we define $f
\extension\ \singleton{n} = \{(x, n) \mapsto f(x) \stt x \in
X\}$ as the function extending $f$ to $X \times
\singleton{n}$; analogously, for a relation $R \subseteq X \times
Y$, we let $R \extension\ \singleton{n} = \{((x, n), (y,n)) \stt (x,y)
\in R\}$ be the relation extending $R$ to $(X \times \singleton{n})
\times (Y \times \singleton{n})$.

We now define two important constructions to compose pomsets
in parallel and sequentially.

%
\begin{definition}
  Let $\apom=[\eset, \leq, \alf]$ and
  $\apom'=[\eset', \leq', \alf']$ be two pomsets.
  %
  The \emph{parallel composition of $\apom$ and $\apom'$} is:
  %
  \begin{align*}
    \rpar[\apom][\apom'] \quad = \quad [\eset \uplus \eset', \ 
    (\leq \extension\ \singleton{1}) \cup 
    (\leq' \extension\ \singleton{2}),\  
    (\alf \extension\ \singleton{1}) \cup 
    (\alf' \extension\ \singleton{2})]
  \end{align*}
  For a pomset $\apom$ and a participant $\p \in \pset$, let
  $\eset_{\apom, \p} = \{\ae \in \esetof \apom \stt \subject[\alfof
  \apom(\ae)] = \p \}$ be the set of events of $\p$ in
  $\esetof \apom$.
  %
  The \emph{sequential composition of $\apom$ and $\apom'$} is:
		where
		\begin{align*}
		  \eset_{\apom, \p} = & \{\ae \in \esetof \apom \sst
		  \esbj[\alfof \apom(\ae)] = \p\}
		  \\
		  \leq_{seq}\  = &
		  \bigcup_{\p \in \pset}
								 \big((\eset_{r,\p} \times \singleton{1}) \times
								 \big\{(\ae,2) \in \eset_{r',\p} \times \singleton{2} \sst
								 \alf'(\ae) \in \lset^!\big\}\big)^\star
		  \cup
		  (\leq \extension\ \singleton{1}) \cup 
		  (\leq' \extension\ \singleton{2})
		\end{align*}
  \\
  and $\star$ is the reflexive-transitive closure.
\end{definition}
Both parallel and sequential composition preserve the causal
dependencies of its constituents $\leq$ and $\leq'$.
%
However, while there is no new dependency introduced by the parallel
composition, the sequential composition of two pomsets adds to those
in $\leq$ and $\leq'$ the dependencies among events in $\apom$ and
$\apom'$ with the same subject.
%
Basically, a causal relation is induced whenever a participant
performing a communication in $\apom$ also performs a
communication in $\apom'$.

% \begin{definition}\label{def:wellpar} Pomsets $\apom=[\eset, \leq, \alf]$ and
%   $\apom'=[\eset', \leq', \alf']$ are \emph{well-forked} if
%   \begin{align*}
%     \alf(\eset) \cap \alf'(\eset') \cap \lset^? = \emptyset
%   \end{align*}
%   We write $\wellpar[\apom][\apom']$ when $\apom$ and $\apom'$ are
%   well-forked and, for $\aG,\aG' \in \gset$, $\wellpar$ when
%   $\gsem \neq \rbot \land \gsem[\aG'] \neq \rbot \land \forall \apom
%   \in \gsem[\aG], \apom' \in \gsem[\aG'] \qst \wellpar[\apom][\apom']$
% \end{definition}

% \begin{definition}\label{def:wellseq} Pomsets $\apom=[\eset, \leq, \alf]$ and
%   $\apom'=[\eset', \leq', \alf']$ are \emph{well-sequenced} if
% \begin{align*}
% \leqof{\rseq[\apom][\apom']} \quad \supseteq \quad 
% (\{\ae \in \eset \stt \alf(\ae) \in \lset^!\} \times \singleton{1})
% \times (\{\ae \in \eset' \stt \alf'(\ae) \in \lset^?\} \times \singleton{2})
% \end{align*}
% We write $\ws[\apom][\apom']$ when $\apom$ and $\apom'$ are
% well-sequenced and, for $\aG,\aG' \in \gset$, $\ws$ when
% $\gsem \neq \rbot \land \gsem[\aG'] \neq \rbot \land \forall \apom \in \gsem[\aG],
% \apom' \in \gsem[\aG'] \qst \ws[\apom][\apom']$.
% \end{definition}

% The definition of well-branchedness relies on the notions of
% \emph{active} and \emph{passive} participants (defined
% in~\cite{tuosto:jlamp-95}) that single out those participants that
% (internally) select which branch to execute and those participants
% that have to \quo{understand} what choice was made according to the
% messages they receive, instead of internally choosing a branch.
% \begin{definition}
% Two g-choreographies $\aG$ and $\aG'$ are \emph{well-branched} when
% \begin{itemize}
% \item[($i$)] there is at most one \emph{active} participant in
%   $\gcho[]$ and
% \item[($ii$)] all the other participants of $\gcho[]$ are
%   \emph{passive}.
% \end{itemize}
% We write $\wb$ to denote that $\aG$ and $\aG'$ are well-branched.
% \end{definition}

For the sake of this paper, We restrict to well-formed~\cite{tuosto:jlamp-95} g-choreographies
for which the semantics is:
\begin{definition}[Semantics of g-choreography]
  The semantics of g-choreographies is
% by the partial map $\gsem[\_][{\nmerge[][]}] : \gset \to \parts{(\parts{\eset}   \times \parts{\eset})}$ below\footnote{We assume $\nmerge[][]$ to be understood and simply write $\gsem[\_]$.}:
\begin{align*}
  \gsem[\gempty] & = \{\emptypom\}
  \\
  \gsem[{\gint[]}] & = \{ [\big(\{\ae_1, \ae_2\},
                       \{(\ae_1,\ae_1), (\ae_2, \ae_2), (\ae_1, \ae_2)\},
                     \alf \big)] \} \text{ where } \alf : \begin{cases} \ae_1 \mapsto \aout \\ \ae_2 \mapsto \ain \end{cases}
  \\
  \gsem[{\gpar[]}] & = 
      \{\rpar[\apom][\apom'] \stt (\apom, \apom') \in {\gsem[\aG]} \times {\gsem[\aG']} \}
  \\
  \gsem[{\gseq[]}] & =
      \{\rseq[\apom][\apom'] \stt (\apom, \apom') \in {\gsem[\aG]} \times {\gsem[\aG']}\}
  \\
  \gsem[{\gcho[]}] & =  %\label{seq:cho}
      \gsem[\aG] \cup \gsem[\aG']
\end{align*}
\end{definition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

